The Rashomon Importance Distribution: Getting RID of Unstable, Single Model-based Variable Importance

Quantifying variable importance is essential for answering high-stakes questions in fields like genetics, public policy, and medicine. Current methods generally calculate variable importance for a given model trained on a given dataset. However, for a given dataset, there may be many models that explain the target outcome equally well; without accounting for all possible explanations, different researchers may arrive at many conflicting yet equally valid conclusions given the same data. Additionally, even when accounting for all possible explanations for a given dataset, these insights may not generalize because not all good explanations are stable across reasonable data perturbations. We propose a new variable importance framework that quantifies the importance of a variable across the set of all good models and is stable across the data distribution. Our framework is extremely flexible and can be integrated with most existing model classes and global variable importance metrics. We demonstrate through experiments that our framework recovers variable importance rankings for complex simulation setups where other methods fail. Further, we show that our framework accurately estimates the true importance of a variable for the underlying data distribution. We provide theoretical guarantees on the consistency and finite sample error rates for our estimator. Finally, we demonstrate its utility with a real-world case study exploring which genes are important for predicting HIV load in persons with HIV, highlighting an important gene that has not previously been studied in connection with HIV. Code is available at https://github.com/jdonnelly36/Rashomon_Importance_Distribution.

==> paper_files/introduction.tex <==
% This heading is temporary
%\subsection{A Simple Motivational Example}

% Why are researchers interested in variable importance? Is it to study a particular model or set of models? Or is the goal to learn about a dataset? Or, better yet, the distribution the dataset comes from? While there is value in each of these goals, we propose that the ultimate goal of studying variable importance is to better understand the distribution from which a dataset is drawn. Unfortunately, this is difficult because researchers only have a finite dataset, which restricts us to limited model classes since overly expressive models will over fit the observed data. This leads the question that we aim to answer in this work: within the limits of a finite dataset and a restricted model class, what can we say about the importance of a variable across the distribution of data?

%The ability to extract the importance of a variable to the underlying data distribution has important implications in domains such as . 
The ability to automatically determine feature importance allows researchers to guide the exploration of subcomponents of complex, real-world systems. These insights are particularly important when studying systems with complicated underlying mechanisms such as genetics  \citep{wang2020initial, novakovsky2022obtaining}, finance \citep{bracke2019machine, rudin2019we}, and criminal justice \citep{FisherRuDo19, propublica}. Prior work has largely approached this problem by developing a single model or algorithm, and analyzing variable importance of the model as if it represents that of the underlying data distribution. However, there are often many very different models that explain a given dataset's behavior equally well \citep{breiman2001statistical, semenova2022existence}, a phenomenon referred to as the Rashomon effect. To account for the Rashomon effect, \cite{FisherRuDo19, dong_exploring_2020} propose variable importance measures that leverage the set of all good models for a dataset. However, \cite{FisherRuDo19} provided only a range of variable importance, and \cite{dong_exploring_2020} proposed looking at \textit{all} of the variable importances for a dataset; neither provided any concrete information about the true variable importance for the underlying distribution of data.
In fact, these works recognized that because of finite sample biases, the set of models explaining a single dataset may still not generalize well to the underlying distribution of data, and therefore made no conclusions about it. When researchers do not account for both the Rashomon effect and finite sample biases, it is possible for two independent researchers to draw very different conclusions about a single phenomenon. The question is whether we can do better than either making the assumption that a single model's importance represents the true importance, or simply making no conclusion.


%Consider the following example: given boolean features $X^{(1)}$ and $X^{(2)}$, we define outcome $Y$ as ``$Y= X^{(1)} \text{ or } X^{(2)}$,'' as shown in Table \ref{tab:toy_dgp} (Left). We draw a dataset of three samples from this population, illustrated in Table \ref{tab:toy_dgp} (Center). There are two models that explain the dataset shown in Table \ref{tab:toy_dgp} (Center) equally well (as measured by accuracy): $f_1,$ which is defined as ``$Y=X^{(1)} \text{ or } X^{(2)}$,'' and $f_2$ which is defined as ``$Y = X^{(1)}$.''
% $f_1$, which is defined as ``$Y = X^{(1)}$,'' and $f_2$, which is defined as ``$Y=X^{(1)} \text{ or } X^{(2)}$''. 
%If we relied solely on $f_2$ as an explanation for this data distribution, we would (incorrectly) conclude that only $X^{(1)}$ matters for predicting the outcome $Y$; if we extract $f_1$, we would (correctly) conclude that both $X^{(1)}$ and $X^{(2)}$ matter for predicting $Y$. Both models are equally good for our observed data, yet they lead to dramatically different insights into the underlying data distribution. \textit{By using a variable importance metric that is tied to a specific model, we limit our ability to gain insight into all good explanations for this dataset.} 

%\begin{table*}[h!]
%    \centering
%    \begin{tabular}{c|c|c|c}
%         & $X^{(1)}$ & $X^{(2)}$ & $Y$ \\
%         \hline
%       1 &  0   &  0   &  0  \\
%       2 &  1   &  0   &  1  \\
%       3 &  0   &  1   &  1  \\
%       4 &  1   &  1   &  1  
%    \end{tabular}
%    \hspace{0.1\linewidth}
%    \begin{tabular}{c|c|c|c}
%         & $X^{(1)}$ & $X^{(2)}$ & $Y$ \\
%         \hline
%       1 &  0   &  0   &  0  \\
%       2 &  1   &  0   &  1  \\
%       & & & \\
%       4 &  1   &  1   &  1  
%    \end{tabular}
%    \hspace{0.1\linewidth}
%    \begin{tabular}{c|c|c|c}
%         & $X^{(1)}$ & $X^{(2)}$ & $Y$ \\
%         \hline
%       1 &  0   &  0   &  0  \\
%       & & & \\
%       3 &  0   &  1   &  1  \\
%       4 &  1   &  1   &  1  
%    \end{tabular}
%    \caption{These tables describe data drawn from a hypothetical data generating process with two binary features $X^{(1)}$ and $X^{(2)}$ and binary outcome $Y = X^{(1)} \lor X^{(2)}.$ Left: The population from which samples are drawn, following this data generating process. Center: A three sample dataset drawn from the population. Right: An alternative three sample dataset drawn from the population.}
%    \label{tab:toy_dgp}
%\end{table*}
%
%\begin{table}
%    \centering
%    \begin{tabular}{l|c|c|c}
%         & $X^{(1)}$ & $X^{(2)}$ & $Y$ \\
%         \hline
%       1 &  0   &  0   &  0  \\
%       2 &  1   &  0   &  1  \\
%       4 &  1   &  1   &  1  
%    \end{tabular}
%    \caption{This table describes a hypothetical \textit{dataset} in which observations were sampled from the data generating process described in Table \ref{tab:toy_dgp}.}
%    \label{tab:toy_dataset1}
%\end{table}


%Now imagine that we draw a different set of three samples from this data generating process, resulting in the dataset shown in Table \ref{tab:toy_dgp} (Right). In this case, we might extract the two equally strong models $f_1$, which is again defined as ``$Y=X^{(1)} \text{ or } X^{(2)}$'', and $f_3$, which is defined as $Y=X^{(2)}$. We can see that $f_1$ is a strong explanation for both datasets, but without considering both sampled datasets we cannot determine which of $f_1, f_2, f_3$ best explain the underlying data distribution. \textit{By using a variable importance metric that is tied to a single dataset and a single model, we limit our ability to draw insights on the underlying distribution of the data.}

We face two key sources of uncertainty in estimating variable importance: modeling uncertainty, which stems from measuring variable importance on a single model, and sampling uncertainty, which stems from usng a single dataset. 
%\textit{By using a variable importance metric that is tied to a specific model, we limit our ability to gain insight into all good explanations for this dataset.}
%\textit{By using a variable importance metric that is tied to a single dataset and a single model, we limit our ability to draw insights on the underlying distribution of the data.}
%This example demonstrates that we must consider all good models across many datasets in order to understand the mechanisms driving this system. 
In this work, we address these issues by introducing the \textit{Rashomon Importance Distribution} ($\ourvi$), which quantifies the distribution of variable importance for all good models across many datasets. We utilize a bootstrap algorithm to overcome sampling biases and use recent advancements in calculating the Rashomon set of optimal sparse decision trees \citep{xin2022exploring} to account for the Rashomon effect. In doing so, we can characterize variable importance for the underlying data distribution in a way that is both stable and robust in the sense of \cite{yu2013stability}.
% In \ourvi, we compute the distribution of variable importance across the Rashomon set for many bootstrap samples of a representative dataset. 

Our contributions are threefold. First, we propose a new variable importance estimand that expands previous variable importance metrics to account for both sampling biases and the Rashomon effect. We also present a bootstrap-style estimation strategy for our estimand. 
Second, we analytically derive error bounds for our methodology and show through synthetic experiments that $\ourvi$ better captures variable importance for the data generating process (DGP) than previous work. 
Finally, we highlight the utility of our method through a criminal justice case study, finding that age is a significant driver of recidivism over the time period and location where our data were collected.

The rest of this work is structured as follows. In Section \ref{sec:related_work}, we provide an overview of prior work studying variable importance and the Rashomon effect. Section \ref{sec:methods} introduces the \ourvi framework and estimation strategy. In Sections \ref{subsec:recovering-rankings} and \ref{subsec:recovering-values}, we use synthetic datasets to demonstrate (1) that \ourvi recovers the ranking of variable importance for the underlying data distribution and (2) that \ourvi captures the true value of the model reliance 
%VI 
metric for the underlying data distribution. Having validated \ourvi against known data distributions, we conduct a case study using \ourvi to measure which factors are important for predicting recidivism in Section \ref{sec:case_study}. Finally, we summarize our findings and underscore our contributions to the literature in Section \ref{sec:conclusion}. 



%\begin{table}[h]
%    \centering
%    \begin{tabular}{l|c|c|c}
%         & $X^{(1)}$ & $X^{(2)}$ & $Y$ \\
%         \hline
%       1 &  0   &  0   &  0  \\
%       3 &  0   &  1   &  1  \\
%       4 &  1   &  1   &  1  
%    \end{tabular}
%    \caption{This table describes another hypothetical \textit{dataset} in which observations were sampled from the data generating process described in Table \ref{tab:toy_dgp}.}
%    \label{tab:toy_dataset2}
%\end{table}



==> paper_files/introduction2.tex <==
Variable importance enables researchers to investigate how different mechanisms interact with each other to draw insights about complex, real world systems. These insights are particularly important in high stakes, intricate real world domains such as genetics  \citep{wang2020initial, novakovsky2022obtaining}, finance \citep{bracke2019machine, rudin2019we}, and criminal justice \citep{FisherRuDo19, propublica}. Prior work has largely approached this problem by developing a single model or algorithm, and analyzing variable importance for the model as if it represents that of the underlying data distribution. However, the efficacy of these variable importance measurements is often limited by two forms of uncertainty: sampling uncertainty and the Rashomon effect.
% These approaches assume that the model produced for the observed dataset perfectly reflects the underlying data distribution. In practice, this is almost never the case due to a combination of sampling uncertainty and modeling uncertainty. 

%However, these variable importance measurements are often influenced by perturbations to a dataset (e.g., bootstrapping) -- referred to as stability -- or perturbations to the model of interest -- referred to as robustness \cite{yu2013stability}. Without considering stability and robustness, we could not guarantee that the variable importance measured gathered on the single dataset and the single model generalize to other datasets.

Firstly, sampling uncertainty leads to biased decision-making because statistics computed on observed data are not necessarily guaranteed to generalize to other, unobserved datasets. To overcome this issue, frequentist statistics quantify how well a statistic computed on a single model and dataset generalizes to that same model for the population using confidence intervals or $p$-values. Secondly, the Rashomon effect --  a phrase coined by Leo Breiman \citep{breiman2001statistical} -- describes the phenomenon in which multiple models that describe a dataset equally well lead to differing insights. To overcome this issue, machine learning researchers have developed methods to compute the Rashomon set -- the set of all near-optimal models -- for a given dataset, enabling us to consider the entire set of good models for that dataset rather than subscribing to a single model.

In this work, we present a framework unifying traditional concepts from Frequentist statistics with recent developments on Rashomon sets to overcome the limitations of traditional variable importance measurements. We propose a model-agnostic estimand for quantifying variable importance while overcoming modeling and sampling uncertainty and a corresponding bootstrap-style estimation strategy. Further, we analytically derive error bounds for our estimates and demonstrate through experiments that our estimand better characterizes feature importances for the data generating process (DGP) than previous work. Lastly, we highlight the utility of our method through a case study in criminal justice, demonstrating that age is a significant predictor of recidivism.

% The rest of this work is structured as follows. In Section \ref{sec:related_work}, we provide an overview of prior work studying variable importance and the Rashomon effect. Section \ref{sec:methods} introduces the \ourvi framework and estimation strategy. In Sections \ref{subsec:recovering-rankings} and \ref{subsec:recovering-values}, we use synthetic datasets to demonstrate (1) that \ourvi recovers the ranking of variable importance for the underlying data distribution and (2) that \ourvi captures the true value of the model reliance VI metric for the underlying data distribution. Having validated \ourvi against known data distributions, we conduct a case study using \ourvi to measure which factors are important for predicting recidivism in Section \ref{sec:case_study}. Finally, we summarize our findings and underscore our contributions to the literature in Section \ref{sec:conclusion}. 

==> paper_files/latexmkrc <==
# This shows how to use the xr package with latexmk.
# John Collins 2023-03-29
#
# The xr package ("a system for eXternal References") is used by a document
# to make references to sections, equations, etc in other external
# documents. 
# The definitions in this file enable latexmk to apply latexmk to
# automatically update an external document whenever its .tex file changes,
# so that the references in the main document stay up to date.

# Notes:
#    1. This version is defined to put the files from the compilations of
#       the external documents into a defined subdirectory, to segregate
#       potentially many generated files from the main document
#       directories. 
#    2. But for latexmk's custom dependency mechanism to be used, as here,
#       the aux file from compilation of a subdocument must be generated in
#       the same directory as the corresponding source .tex file.  So the
#       .aux file is copied.
#    3. It is assumed that the external documents are to be compiled by
#       pdflatex.  This can be changed, of course, by changing the '-pdf'
#       option given to the invoked latexmk to whatever is needed.
#    4. An ideal implementation would also ensure that recompilation of an
#       external document also happens whenever any of its other source
#       files changes.  But this is not done in the present version, and
#       would probably entail either the use of internal latexmk variables
#       or extra enhancements to latexmk.
#    5. The code uses subroutines copy and fileparse that are loaded by
#       latexmk from the Perl packages File::Copy and File::Basename.
#    6. It also uses some not-yet-documented features of latexmk: an array
#       variable @file_not_found and subroutines popd, pushd, and
#       rdb_add_generated. 


#--------------------
# Configurable choices for compilation of external documents

# Subdirectory for output files from compilation of external documents:
$sub_doc_output = 'output-subdoc';

# Options to supply to latexmk for compilation of external documents:
@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

#--------------------

# Add a pattern for xr's log-file message about missing files to latexmk's
# list.  Latexmk's variable @file_not_found is not yet documented.
# This line isn't necessary for v. 4.80 or later of latexmk.
push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {
               # In this case, .aux file generated by pdflatex isn't in same
               # directory as the .tex file.
               # Therefore:
               # 1. Actual generated aux file must be listed as produced by this
               #    rule, so that latexmk deals with dependencies correctly.
               #    (Problem to overcome: If $sub_dir_output is same as $aux_dir
               #    for the main document, xr may read the .aux file in the
               #    aux_dir rather than the one the cus dep is assumed by latexmk
               #    to produce, which is in the same directory as the .tex source
               #    file for this custom dependency.)
               #    Use not-yet-documented latexmk subroutine rdb_add_generated
               #    to do this:
               # 2. A copy of the .aux file must be in same directory as .tex file
               #    to satisfy latexmk's definition of a custom dependency.
             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> paper_files/methods.tex <==
\subsection{Definitions and Estimands} \label{sec:defEstimands}
% Throughout this work, we use the following notation. 
Let $\mathcal{D}^{(n)} = \{(X_i, Y_i)\}_{i=1}^n$ denote a dataset of $n$  independent and identically distributed tuples, where $Y_i\in \mathbb{R}$ denotes some outcome of interest and $X_i\in \mathbb{R}^p$ denotes $p$ covariates. Let $g^*$ represent the data generating process (DGP) producing $\Dn$. Let $f \in \mathcal{F}$ be a model in a model class (e.g., a tree in the set of all possible sparse decision trees), and let $\phi_j\left(f, \mathcal{D}^{(n)}\right)$ denote a function that measures the importance of variable $j$ for a model $f$ over a dataset $\Dn.$ This can be any of the functions described earlier (e.g., permutation importance, SHAP). Our framework is flexible with respect to the user's choice of $\phi_j$ and enables practitioners to use the variable importance metric best suited for their purpose; for instance, conditional model reliance is best-suited to measure only the unique information carried by the variable (that cannot be constructed using other variables), whereas other metrics like subtractive model reliance consider the unconditional importance of the variable. Our framework is easily integrable with either of these.
Finally, let $\ell(f, \Dn; \lambda)$ represent a loss function given $f, \Dn,$ and loss hyperparameters $\lambda$ (e.g., regularization).  We assume that our loss function is bounded above and below, which is true for common loss functions like 0-1 classification loss, as well as for differentiable loss functions with covariates from a bounded domain. Additionally, assume that the variable importance function $\phi$ has a bounded, non-negative range.
%, which holds for many metrics like conditional model reliance. 

%\begin{assumption}
%The loss function is bounded: there exist some constants $\ell_{\min}$ and $\ell_{\max}$ such that $\ell_{\min} \leq \ell(f, \Dn; \lambda) \leq \ell_{\max}$ for all values $f$, $\Dn$, and $\lambda$.
%\end{assumption}
%\begin{assumption}
%    The variable importance function is bounded: there exist constants $\phi_{\min}$ and $\phi_{\max}$ such that $0 \leq \phi_{\min} \leq \phi_j\left(f, \mathcal{D}^{(n)} \right) \leq \phi_{\max}$ for all values $f$, $\Dn$, and $j = 1, \ldots, m$. 
%\end{assumption}


% Ideally, we would account for sampling uncertainty and compute variable importance directly on the DGP $g^*$ by calculating a variable importance distribution ($VID$) for each possible datasets $\Dn$:
% \begin{align*}
%     \mathbb{P}(VID \leq k) = \mathbb{E}_{\Dn}\left[ \mathbb{1}[\phi_j(g^*, \Dn) \leq k] \right].
% \end{align*}
% However, $g^*$ is unknown in practice.
In an ideal setting, we would measure variable importance using $g^*$ and the whole population, but this is impossible because $g^*$ is unknown and data is finite. 
% Given infinite data, we would measure the importance of variables for the DGP $g^*,$ but $g^*$ is unknown and we do not have infinite data in practice. 
In practice, scientists instead use the empirical loss minimizer for a specific dataset $\hat{f}^* \in \arg\min_{f \in \mathcal{F}} \ell(f, \Dn)$ as a surrogate for $g^*$; however, several models could explain the same dataset equally well (i.e., the Rashomon effect). Rather than using a single model as a surrogate for $g^*,$ we propose to use the entire Rashomon set to quantify variable importance.
% We represent the importance of a given feature across (1) the set of good explanations for each $\Dn$ (i.e., the Rashomon set) and (2) the distribution that generates all datasets of size $n$.
Given a single dataset $\Dn$, we define the Rashomon set for a model class $\mathcal{F}$ and parameter $\varepsilon$  as the set of all models in $\mathcal{F}$ whose empirical losses are within some bound $\varepsilon > 0$ of the empirical loss minimizer:
\begin{align} \label{eqn:Rset} \tag{Rashomon Set}
    \mathcal{R}(\epsilon, \mathcal{F}, \ell, \Dn, \lambda) = \left\{ f \in \mathcal{F} : \ell(f, \Dn; \lambda) \leq \min_{f' \in \mathcal{F}} \ell(f', \Dn; \lambda) + \varepsilon \right\}.
\end{align}
We denote this Rashomon set by $\mathcal{R}^{\varepsilon}_{\Dn}$ or ``Rset'' (this assumes a fixed $\mathcal{F}$ and $\lambda$). 
As discussed earlier, the Rashomon set can be fully computed and stored for non-linear models (e.g., sparse decision trees \citep{xin2022exploring}). For notational simplicity, we often omit $\lambda$.

%While prior work chooses $\varepsilon$ arbitrarily, we introduce a principled method for doing so by computing the tightest value $\varepsilon$ that guarantees that the population minimizer is contained within the Rashomon set of an arbitrary dataset of size $n$, $\mathcal{R}(\Dn, \varepsilon, \mathcal{F}, \ell; \lambda ),$ with high probability.
% Theorem \ref{thm:epsilon_bound} introduces a method for choosing $\varepsilon$ such that $f^* \in \mathcal{R}\left(\Dn, \varepsilon, \mathcal{F}, \ell; \lambda\right)$ with high probability.

%\begin{proposition}
%\label{thm:epsilon_bound}
%    Let $\delta \in (0, 1)$, and let $h$ denote some function (e.g., a generalization bound) such that for all $f \in \mathcal{F}$, we have:
%    \begin{align*}
%        \mathbb{P}\left(|\ell(f) - \hat{\ell}(f)| \leq h(\mathcal{F}, n, \delta, \ell; \theta)\right) \geq 1 - \delta ,
%    \end{align*}
%    where $\theta$ denotes some additional parameters. Then, \textcolor{red}{with probability at least $1 - \delta$ with respect to the random draw of data from the DGP},
%    \begin{align}
%        f^* \in \mathcal{R}\left(D^{(n)}, \varepsilon_h, \mathcal{F}; \lambda \right),
%    \end{align}
%    for any $\varepsilon_h \geq 2h(\mathcal{F}, n, \delta, \ell; \theta).$
%    
%\end{proposition}
%%\begin{theorem}
%\label{thm:epsilon_bound}
%    Let $\sigma^2$ be an upper bound on the variance of $\ell$, let $\mathcal{F}$ be a finite model class (e.g., decision trees), and let $c:=\frac{\ell_{\text{max}} - \ell_{\text{min}}}{2}$. For any value $\delta \in (0, 1)$, 
%        \begin{align*}
%            \mathbb{P}(f^* \in \mathcal{R}^{\epsilon_n}_{\Dn}) \geq 1-\delta \text{ for any }
%        \varepsilon_n \geq  \frac{ \frac{-2c}{3}\ln\left(\frac{\delta}{2|\mathcal{F}|} \right) + \sqrt{\frac{4c^2}{9}\ln^2\left(\frac{\delta}{2|\mathcal{F}|} \right)  - 8n\sigma^2\ln\left(\frac{\delta}{2|\mathcal{F}|} \right)}}{2n}.
%    \end{align*}
%\end{theorem}
% NOTE: We are now moving from established definitions to our methods -- we need to motivate each step a bit more.
% I think we should 1) (re)visit our toy example here to directly motivate our stuff. We could say something like:
% " Consider again example 1.blah. As we demonstrated, even in this simple setting, applying $\phi$ to a single model may lead to misleading explanations for the dataset. We propose to address this problem by considering the distribution of $\phi$ across all good models, capturing all viable explanations for this dataset. Given a $\mathcal{D}^{(n)} and \mathcal{R}$, a natural definition for this distribution, referred to as RI, is:
%$ stuff$
% This is good in that... However, this definition faces two major limitations:"
% Then go into our method
% END NOTATION SECTION
%Thus, we can choose $\varepsilon = 2h(\mathcal{F}, n, \delta, \ell; \theta)$ to probabilistically guarantee that the true best-in-class model is in the Rashomon set.
%Proposition \ref{thm:epsilon_bound} can be used with many generalization bounds, including VC bounds, Rademacher complexity bounds, covering number bounds,  or Occam's Razor bounds. %\textcolor{red}{Explicit values for $\varepsilon$ under some common bounds are derived in the appendix.}

While the Rashomon set describes the set of good explanations for a \textit{single} dataset, Rashomon sets vary across permutations (e.g., subsampling and resampling schemes) of the given data. We define a stable quantity for variable importance that accounts for all good models, the \textit{Rashomon Importance Distribution} ($\ourvi$), whose cumulative distribution function (CDF) is defined as follows:  
\begin{align} \label{eq:RID}
    F_{\ourvi_j}(k) &= \mathbb{P}(\ourvi_j(\varepsilon, \mathcal{F}, \ell; \lambda) \leq k)  := \mathbb{E}_{\Dn \sim \mathcal{P}_n}\left[\frac{|\{f \in \mathcal{R}^{\varepsilon}_{\Dn} : \phi_j(f, \Dn) \leq k\}|}{|\mathcal{R}^{\varepsilon}_{\Dn}|} \right]\\
    &= \mathbb{E}_{\Dn \sim \mathcal{P}_n}\left[\frac{\textrm{volume of Rset where variable $j$'s importance is at most $k$}}{\textrm{volume of Rset}}\right], \nonumber
\end{align}
where $\phi_j$ denotes the variable importance metric being computed on variable $j$, $k \in [\phi_{\min}, \phi_{\max}]$; for a continuous model class (e.g., linear regression models), the cardinality in the above definition becomes the volume under a measure on the function class, usually $\ell_2$ on parameter space. \ourvi constructs the cumulative distribution function (CDF) for the distribution of variable importance across Rashomon sets; as $k$ increases, the value of $\mathbb{P}(\ourvi_j(\varepsilon, \mathcal{F}, \ell; \lambda) \leq k)$ becomes closer to 1. The probability and expectation are taken with respect to datasets of size $n$ sampled from the empirical distribution $\mathcal{P}_n$, which is the same as considering all possible resamples of size $n$ from the originally observed dataset $\Dn$.
Equation (\ref{eq:RID}) weights the contribution of 
$\phi_j(f, \mathcal{D}^{(n)})$ for each model $f$ by the proportion of datasets for which this model is a good explanation (i.e., in the Rashomon set). Intuitively, this provides greater weight to the importance of variables for stable models.

From $\ourvi$, we can also define the \textit{joint} CDF of importance for each variable, referred to as the Joint Rashomon Importance Distribution (\JRID{}):
\begin{align}
\label{eq:RID_def}
    F_{\JRID{}}(k) &= \mathbb{P}\left(\JRID \leq \mathbf{k} \right) := \mathbb{P}(\ourvi_1(\varepsilon, \mathcal{F}, \ell; \lambda) \leq k_1, \ldots, \ourvi_p(\varepsilon, \mathcal{F}, \ell; \lambda) \leq k_p) \\\nonumber
    &= \mathbb{E}_{\Dn}\left[\frac{|\{f \in \mathcal{R}^{\varepsilon}_{\Dn} :  \phi_1(f, \Dn) \leq k_1, \ldots, \phi_p(f, \Dn) \leq k_p \}|}{|\mathcal{R}^{\varepsilon}_{\Dn}|} \right],
\end{align}
where $\mathbf{k} = [k_1, \ldots, k_p] \in [\phi_{\min}, \phi_{\max}]^p$. 
We also define an analogous metric for the loss function $\ell$; we define the Rashomon loss distribution (\RLD{}) as the expected fraction of functions in the Rashomon set where the loss is smaller than $k$.
\begin{align*}
    \mathbb{P}\left(\RLD{}(\varepsilon, \mathcal{F}, \ell; \lambda) \leq k\right) &:= \mathbb{E}_{\Dn}\left[\frac{|\{f \in \mathcal{R}^{\varepsilon}_{\Dn} : \ell(f, \Dn) \leq k \} |}{|\mathcal{R}^{\varepsilon}_{\Dn}|} \right] \\
    &= \mathbb{E}_{\Dn}\left[\frac{|\mathcal{R}\left(k - \min_{f \in \mathcal{F}}\ell(f, \Dn), \mathcal{F}, \ell; \lambda\right)|}{|\mathcal{R}(\varepsilon, \mathcal{F}, \ell; \lambda)|} \right].
\end{align*}
This quantity shows how quickly the Rashomon set fills up on average as loss changes. If there are many near-optimal functions, this will grow quickly with $k$.

In order to connect \JRID{} for model class $\mathcal{F}$ to the unknown DGP $g^*$, we make a Lipschitz-continuity-style assumption on the relationship between \RLD{} and $\JRID{}$ relative to a general model class $\mathcal{F}$ and $\{g^*\}.$  To draw this connection, we define the loss CDF for $g^*$, called $LD^*$, over datasets of size $n$ as:
\begin{align*}
    \mathbb{P}(LD^*(\ell, n; \lambda) \leq k) := \mathbb{E}_{\Dn} \left[\mathbb{1}[\ell(g^*, \Dn) \leq k]\right].
\end{align*}
One could think of $LD^*$ as measuring how quickly the DGP's Rashomon set fills up as loss changes. Here, $LD^*$ is the analog of \RLD{} for the data generation process.

% \begin{assumption} \label{asm:lipschtiz}
%     If $|RLD(\varepsilon, \mathcal{F}, \ell;\lambda)  - 
%      RLD(\ell_{\max}, \{g^*\}, \ell;\lambda) | < \gamma,$ then for $q \in [0, 1],$ the following is true:
%     \begin{align*}
%         \left| Q_{\ourvi(g^*)}(q) - Q_{\ourvi(\mathcal{F})}(q) \right| < d(\gamma)
%     \end{align*}
%     for a monotonically increasing, affine, invertible function $d: \mathbb{R}^+ \to \mathbb{R}^+.$ Here, $Q_{\ourvi(F)}(q)$ represents the $q$-th quantile of $\ourvi$ for the model class $\mathcal{F}.$
% \end{assumption}

\begin{assumption} \label{asm:lipschitz}
    Let $d$ be a monotonically increasing, affine, invertible function $d: [0, \ell_{\max} - \ell_{\min}] \to [0, \phi_{\max} - \phi_{\min}].$ Let $\rho$ represents any distributional distance metric (e.g., 1-Wasserstein).
    If 
    \begin{align*}
        \rho\left(\RLD(\varepsilon, \mathcal{F}, \ell;\lambda),
     LD^*(\ell, n;\lambda) \right) &\leq \gamma \text{ then } \\
        \rho\left(\JRID(\varepsilon, \mathcal{F}, \ell; \lambda), \JRID(\varepsilon, \{g^*\}, \ell ; \lambda) \right) &\leq d(\gamma)
    \end{align*}
    %for a monotonically increasing, affine, invertible function $d: [0, \ell_{\max} - \ell_{\min}] \to [0, \phi_{\max} - \phi_{\min}].$ Here, $\rho$ represents any distributional distance metric (e.g., 1-Wasserstein).
\end{assumption}

Assumption \ref{asm:lipschitz} says that a Rashomon set consisting of good approximations for $g^*$ in terms of loss will also consist of good approximations for $g^*$ in terms of variable importance; i.e., loss is smooth in variable importance. 
More formally, from this assumption, we know that as $\rho(LD^*, \RLD) \to 0$, the joint variable importance distributions will converge: $\rho\left(\JRID(\varepsilon, \mathcal{F}, \ell; \lambda), \JRID(\varepsilon, \{g^*\}, \ell ; \lambda) \right) \to 0.$ We demonstrate that this assumption is realistic for a variety of model classes like linear models and generalized additive models in Section C of the supplement.

% We prove that computing the $\alpha$-central credible region of $\ourvi$ contains the median of $VID$ with high probability. 

% We demonstrate that as the predictive performance of the Rashomon set for a model class $\mathcal{F}$ converges to the predictive performance of the DGP $g^*$, the probability of the $\alpha$-central credible region (CCR) of $\ourvi$ for $\mathcal{F}$ covering the median of $\ourvi$ when the model class is just $\{g^*\}$ also increases.

\subsection{Estimation}
We estimate both $\ourvi_j$ for each variable $j$ and the joint distribution across all variables ($\JRID{}$) by leveraging bootstrap sampling to draw new datasets from the empirical data distribution: we sample observations from an observed dataset, construct its Rashomon set, and compute the $j$-th variable's importance for each model in the Rashomon set. After repeating this process for $B$ bootstrap iterations, we estimate the Rashomon Importance Distribution by weighting each model $f$'s realized variable importance score by the proportion of the bootstrapped datasets for which $f$ is in the Rashomon set \textit{and} the size of each Rashomon set in which $f$ appears.
%
Specifically, let $\Dn_b$ represent the dataset sampled with replacement from $\Dn$ in iteration $b = 1, \ldots, B$ of the bootstrap procedure. For each dataset $\Dn_b$, we find the Rashomon set $\mathcal{R}_{\Dn_b}^{\varepsilon}$. We then estimate $\JRID{}$ by computing
\begin{align}
    \mathbb{P}(\widehat{\JRID{}}(\varepsilon, \mathcal{F}, \ell; \lambda) \leq \mathbf{k}) 
  = \frac{1}{B} \sum_{b=1}^B\left(\frac{|\{f \in \mathcal{R}^{\varepsilon}_{\Dn_b} :  \phi_1(f, \Dn_b) \leq k_1, \ldots, \phi_p(f, \Dn_b) \leq k_p \}|}{|\mathcal{R}^{\varepsilon}_{\Dn_b}|} \right), \notag
\end{align}

and, similarly, estimate $\ourvi_j$ by computing
\begin{align}
    \mathbb{P}(\widehat{\ourvi}_j(\varepsilon, \mathcal{F}, \ell; \lambda) \leq k) 
  = \frac{1}{B}\sum_{b = 1}^B \left(\frac{|\{f \in \mathcal{R}^{\varepsilon}_{\Dn_b} : \phi_j(f, \Dn_b) \leq k \}|}{|\mathcal{R}^{\varepsilon}_{\Dn_b}|} \right). \notag
\end{align}

We can directly connect our estimate $\widehat{\JRID{}}(\varepsilon, \mathcal{F}, \ell; \lambda)$ to the DGP's variable importance distribution $\JRID{}(\ell_{\text{max}}, \{g^*\}, \ell; \lambda)$, which Theorem \ref{thm:wasser} formalizes.

\begin{theorem} \label{thm:wasser}
    Let Assumption \ref{asm:lipschitz} hold for distributional distance $\rho(A_1, A_2)$ between distributions $A_1$ and $A_2$.
    For all $t > 0$, as  $\rho\left(LD^*(\ell, n; \lambda), \RLD(\varepsilon, \mathcal{F}, \ell; \lambda) \right) \to 0$ and $B \to \infty$,
    %Then we have the following result:
    \begin{align*}
        \mathbb{P}\left( \left| \mathbb{P}(\widehat{\JRID{}}(\varepsilon, \mathcal{F}, \ell; \lambda) \leq \mathbf{k}) - \mathbb{P}(\JRID{}(\varepsilon, \{g^*\}, \ell; \lambda) \leq \mathbf{k}) \right| \geq t \right) \to 0
    \end{align*}
\end{theorem}

For a set of models that performs sufficiently well in terms of loss, $\widehat{\JRID{}}$ thus recovers the joint CDF of variable importance for the true model across all reasonable perturbations. In practice, we often care about investigating the importance of a specific variable; because we can recover the joint CDF of variable importance, we guarantee recovery of each marginal CDF. We can even get something stronger than asymptotic convergence: Theorem \ref{thm:ourvi_finite_sample} provides a finite sample bound for the estimation of a marginal distribution. Note that this result does not require Assumption \ref{asm:lipschitz}. 

\begin{theorem} \label{thm:ourvi_finite_sample}
Let $t > 0$ and $\delta \in (0, 1).$ Then, with probability at least $1 - \delta$ with respect to bootstrap samples of size $n$,
\begin{align}
    \left| \mathbb{P}\Big( \widehat{\ourvi}_j(\varepsilon, \mathcal{F}, \ell; \lambda) \leq k \Big) - \mathbb{P}\Big( \ourvi_j(\varepsilon, \mathcal{F}, \ell; \lambda) \leq k \Big) \right| \leq t
\end{align}
with number of bootstrap samples $B \geq \frac{1}{2t^2}\ln\left( \frac{2}{\delta} \right)$ iterations for any $k \in [\phi_{\min}, \phi_{\max}]$.
\end{theorem}

Because we use a bootstrap procedure, we can control the number of bootstrap iterations to ensure that the difference between $\ourvi_j$ and $\widehat{\ourvi}_j$ is within some pre-specified error. (As defined earlier, $\ourvi_j$ is the expectation over infinite bootstraps, whereas $\widehat{\ourvi}_j$ is the empirical average over $B$ bootstraps.) For example, after 471 bootstrap iterations, we find that $\mathbb{P}(\widehat{\ourvi}_j(\varepsilon, \mathcal{F}, \ell; \lambda) \leq k)$ is within 0.075 of $\mathbb{P}(\ourvi_j(\varepsilon, \mathcal{F}, \ell; \lambda) \leq k)$ for any given $k$ with 90\% confidence. It also follows that as $B$ tends to infinity, the estimated $\ourvi_j$ will converge to the true value. %Corollary \ref{cor:ourvi_consistency} states that $\widehat{\ourvi}_j$ is a consistent estimator for $\ourvi_j$.

%\begin{corollary} \label{cor:ourvi_consistency}
%As $B \to \infty,$ 
%\begin{align}
%    \mathbb{P}\left( \left| \mathbb{P}\left( \widehat{\ourvi}_j(\varepsilon, \mathcal{F}, \ell; \lambda) \leq k\right) - \mathbb{P}\left( \ourvi_j(\varepsilon, \mathcal{F}, \ell; \lambda) \leq k \right) \right| \leq \varepsilon \right) = 0.
%\end{align}
%\end{corollary}


% From Theorem \ref{thm:dgp_to_est}, it follows immediately that as $\rho\left(\RLD(\varepsilon_R, \mathcal{F}, \ell;\lambda),
%      RLD(\ell_{max}, \{g^*\}, \ell;\lambda) \right) \to 0$,  

% Finally, we may be interested in arbitrary central credible regions (CCR) of $\ourvi$. 
%Because we can accurately estimate the joint distribution of variable importances $J\ourvi$, it follows that we can accurately estimate the marginal distribution $\ourvi$ for any given variable $j$, which is typically the quantity of interest in practice. We can estimate this quantity as:
%\begin{align}
%    \mathbb{P}(\widehat{\ourvi}_j(\varepsilon, \mathcal{F}, \ell; \lambda) \leq k) 
%  = \frac{1}{B}\sum_{b = 1}^B \left( \frac{\sum_{f \in \mathcal{R}^{\varepsilon}_{\Dn_b}} \mathbb{1}\left[ \phi_j(f, \Dn_b) \leq k \right] }{|\mathcal{R}^{\varepsilon}_{\Dn_b}|} \right). \notag
%\end{align}
%Corollary \ref{cor:ourvi_marginal}, which follows from Theorem \ref{thm:ourvi_finite_sample}, introduces a finite sample bound for estimating $\widehat{\ourvi}_j$.

%\begin{corollary}
%    \label{cor:ourvi_marginal}
%Let $t > 0$ and $\delta \in (0, 1).$ Then, with probability at least $1 - \delta,$
%\begin{align}
%    \left| \mathbb{P}\left( \widehat{\ourvi}_j(\varepsilon, \mathcal{F}, \ell; \lambda) \leq k \right) - \mathbb{P}\left( \ourvi_j(\varepsilon, \mathcal{F}, \ell; \lambda) \leq k \right) \right| \leq t
%\end{align}
%with $B \geq \frac{1}{2t^2}\ln\left( \frac{2}{\delta} \right)$ iterations for any $k$ such that $\phi_{\min} \leq k \leq \phi_{\max}$.
%\end{corollary} 

Since we stably estimate the entire distribution of variable importance values, we can create (1) stable point estimates of variable importance (e.g., expected variable importance) that account for the Rashomon effect (2), interquantile ranges of variable importance, and (3) confidence regions that characterize uncertainty around a point estimate of variable importance. We prove exponential rates of convergence for these statistics estimated using our framework in the supplement.
% The $\alpha CCR$ describes the range of values in  which $100\cdot(1-\alpha)\%$ of a distribution's central mass lies. In a univariate distribution, this quantity can be found using the $\frac{\alpha}{2}$ and $(1 - \frac{\alpha}{2})$ quantiles. The $\tau$-th quantile of a random variable $A$ is the value of $k$ such that $\mathbb{P}(A \leq k) = \tau.$
% Corollary \ref{cor:ccr} provides finite sample bounds for a the region of $\widehat{\ourvi}_j$ that contains a given $\alpha$CCR of $\ourvi_j$ with high probability.
% \begin{corollary}
%     % Let $\varepsilon_H, \delta > 0$. 
%      Let $\alpha \in [0, 0.5]$ be the parameter for some $\alpha$ central credible region ($\alpha CCR$). We define a new robustness region, the estimated coverage region ($ ECR$): given $t > 0,$ let $\tau_{low} = \frac{\alpha}{2} - 2t$ and $\tau_{up} = 1 - \frac{\alpha}{2} + 2t.$ Define 
%     % \begin{align*}
%     $\varepsilon ECR = \left(\hat{Q}_{\tau_{low}}, \hat{Q}_{\tau_{up}} \right),$
%     % \end{align*}
%     where $\hat{Q}_{\tau}$ is the $\tau$-th quantile of $\widehat{\ourvi}_j$. With $B \geq \frac{1}{2t^2} \ln\left( \frac{8}{\delta} \right)$ bootstrap iterations, 
%     \begin{align}
%         \mathbb{P}(\alpha CCR \subseteq ECR) \geq 1 -\delta.
%     \end{align}

% ADD SOME TRANSITION -- "we have shown that we can estimate CCR with this confidence and that $\ourvi$ is consistent; we now proceed to show that this holds experimentally"

    % Let $Q_{\frac{\alpha/2}}$ and $Q_{1 - \frac{\alpha}{2}}$ represent the $\alpha\%-$central credible region in $\ourvi.$ These are the $\frac{\alpha}{2}$ and $100 - \frac{\alpha}{2}$ percentiles in $\ourvi.$ 
    
    % Given quantiles of interest $t_{\text{low}}$ and $t_{\text{up}}$ such that $t_{\text{low}} < t_{\text{up}}$, let $\tau_{\text{low}}:= t_{\text{low}} - 2\varepsilon_H $ and $\tau_{\text{up}}:= t_{\text{up}} + 2\varepsilon_H $. Let $CCR(t_{\text{low}}, t_{\text{high}}):=\mathbb{P}(\ourvi \leq Q_{t_{\text{low}}} ), \mathbb{P}(\ourvi \leq Q_{t_{\text{up}}} )$ denote the region between the $t_{\text{low}}$-th quantile and the $t_{\text{up}}$-th quantile of $\ourvi$, and let $\widehat{CCR}(\tau_{\text{low}}, \tau_{\text{up}}):=\mathbb{P}(\widehat{\ourvi} \leq \hat{Q}_{\tau_{\text{low}}} ), \mathbb{P}(\widehat{\ourvi} \leq \hat{Q}_{t_{\text{up}}} )$ denote the region between the $\tau_{\text{low}}$-th quantile and the $\tau_{\text{up}}$-th quantile of $\widehat{\ourvi}$.
%     Then, with probability at least $1 - 4\delta$,
%     \begin{align*}
%         \left(\mathbb{P}(\ourvi \leq Q_{t_{\text{low}}} ), \mathbb{P}(\ourvi \leq Q_{t_{\text{up}}} )\right)\subseteq \left(\mathbb{P}(\widehat{\ourvi} \leq \hat{Q}_{\tau_{\text{low}}} ), \mathbb{P}(\widehat{\ourvi} \leq \hat{Q}_{\tau_{\text{up}}} )\right)
%     \end{align*}
% with $B \geq \frac{\ln\left( \frac{1 - \delta}{2} \right)}{-2\varepsilon_H^2}$ iterations.
%\label{cor:ccr}
%\end{corollary}

Because our estimand and our estimation strategy (1) enable us to manage instability, (2) account for the Rashomon effect, and (3) are completely model-agnostic and flexibly work with most existing variable importance metrics, $\ourvi$ is a valuable quantification of variable importance. 
% We next demonstrate their empirical performance using synthetic experiments. 

==> paper_files/synthetic_experiments_5_12.tex <==


In this section, we validate $\ourvi$ using four datasets with known data generating processes (DGP's): Monk 1 and Monk 3 \citep{thrun1991monk} \footnote{We exclude Monk 2 from our experiments because there is no clear notion of an expected variable importance ranking for this dataset, since the DGP involves all variables.}, which each follow a distinct non-linear DGP; the non-linear DGP described in \citep{chen2017kernel}, referred to as Chen's dataset; and the non-linear DGP introduced in \cite{friedman1991multivariate}, referred to as Friedman's dataset. 
We first evaluate $\ourvi$'s ability to distinguish between variables that are used by the DGP and those that aren't in \ref{subsec:recovering-rankings}. This experiment allows us to assess the accuracy of each variable importance method without subscribing to a specific metric $\phi$, enabling cross-metric comparisons. We then evaluate $\ourvi$'s ability to recover variable importance \textit{values} for the DGP on a fixed metric $\phi,$ enabling us to assess $\ourvi$'s ability to capture absolute importance. Finally, we demonstrate that $\ourvi$ produces stable inter quantile regions across independent recreations of the Monk 3 dataset, solving the problem of instability in the Rashomon set.


%In both cases, we consider four datasets: Monk 1 and Monk 3 \cite{thrun1991monk}, which each follow a distinct non-linear DGP; and the linear DGP described in \cite{hooker2021unrestricted} both with and without correlation between variables referred to as ``Hooker $(\rho = 0.9)$'' and ``Hooker $(\rho = 0)$'' respectively. We convert the datasets described in \cite{hooker2021unrestricted} into binary classification tasks by setting our label to $1$ if and only if the original outcome is greater than the median. See the Appendix for a more detailed description of the experimental setup.

%\begin{table}[h!]
%    \centering
%    \begin{tabular}{c|c|c}
%        Dataset & Features & DGP  \\
%        \hline
%        Monk 1 & 6 & ($a_1$ = $a_2$) or ($a_5$ = 1)\\
%        Monk 2 & 6 & EXACTLY TWO of:
%        \\&&\{$a_1$ = 1, $a_2$ = 1, 
%        \\&&$a_3$ = 1, $a_4$ = 1,
%        \\&&$a_5$ = 1, $a_6$ = 1\}\\
%        Monk 3 & 6 & (a5 = 3 and a4 = 1) 
%        \\&&or (a5 $\neq$ 4 and a2 $\neq$ 3)\\
%        Hooker & 10 & $a_1 + a_2 + a_3 + a_4$\\
%        &&$ + a_5 + 0a_6 + 0.5a_7$
%        \\&&$ + 0.8a_8 + 1.2a_9 + 1.5a_{10}$
%    \end{tabular}
%    \caption{Overview of the DGP used in our example datasets. In the Monk datasets, $a_1, \ldots, a_6$ take on values $\{1, 2, 3, 4\}$. In the Hooker datasets, $a_1, \ldots, a_{10}$ take on real values between 0 and 1.}
%    \label{tab:dgps}
%\end{table}

Throughout the following sections, we evaluate $\ourvi$ using the Rashomon set of all accurate and sparse decision trees as extracted by the TreeFARMS algorithm of \cite{xin2022exploring}. For all of our experiments, %except for those on the Hooker dataset with $\rho=0.9$, 
we evaluate $\ourvi$ using subtractive model reliance $\phi_{\text{sub}}$ \citep{FisherRuDo19}.
%, defined as
%\begin{align}
%    \label{eq:sub-mr}
%    \phi_{\text{sub}}(f, \mathcal{D}^{(n)}, v) &= \ell_{\text{switch}} - \ell(f, \mathcal{D}^{(n)}),
%\end{align}
%where $\ell$ is $0-1$ misclassification loss function, $\ell_{\text{switch}}$ is defined as
%\begin{align*}
%    \ell_{\text{switch}} &= 
%    \frac{1}{|P(\mathcal{D}^{(n)}, v)|}\sum_{\mathcal{D}_{\text{perm}}^{(n)} \in \mathcal{P}^{(v)}_{\mathcal{D}^{(n)}}} \ell(f, \mathcal{D}_{\text{perm}}^{(n)}),
%\end{align*}
%and $\mathcal{P}^{(v)}_{\mathcal{D}^{(n)}}$ denotes the set of datasets for all permutations of $X_1^{(v)}, X_2^{(v)}, \hdots, X_n^{(v)}$. 
The metric $\phi^{\text{sub}}$ captures how much worse a model performs when the information given by variable $j$ is scrambled, i.e., permuted (so that $j$ becomes noise with the same marginal distribution as variable $j$). 
%In the case of the Hooker dataset with high correlation, we evaluate $\ourvi$ using the conditional model reliance (CMR) metric proposed in \cite{FisherRuDo19} over the 0-1 misclassification loss function. CMR is designed to capture the \textit{unique} information offered by a variable, and as such is expected to perform better in the presence of highly correlated variables.
%. For computational efficiency, we estimate $\ell_{\text{switch}}$ using the $e_{\text{divide}}$ strategy recommended in \cite{FisherRuDo19}. 

\subsection{Recovering Rankings}
\label{subsec:recovering-rankings}

\begin{figure*}[ht]
    \centering
    % \includegraphics[width=0.98\linewidth]{figures/baseline_rankings.png}
    
     \includegraphics[width=1\textwidth]{figures/baseline_rankings_wchen.png}
    \caption{The proportion of features ranked correctly by each baseline model on each data set represented as a \textit{stacked} barplot. The following describes each previously undefined acronym: RF = random forest; LASSO = L1 regularized logistic regression; PDP = partial dependency plots; CMR = conditional model reliance. The figures are ordered according to method performance across the three datasets. $\ourvi$, MR RF, RF Impurity, RF Permute, and VIC recovered rankings perfectly.}
    \label{fig:baseline-rankings}
\end{figure*}


For each dataset evaluated in Figure \ref{fig:baseline-rankings}, we evaluate the ability of each variable importance method to distinguish between variables that are used and not used to generate the outcome.
%=\{ \{(X_i^{(j)}, X_i^{(v)}, Y_i)\}_{i=1}^n \}$
We extract variable importance rankings from $\ourvi$ by evaluating $\ourvi$ for each variable in a given dataset $\Dn$ across $B=500$ bootstrap iterations and estimating $\mathbb{E}[\ourvi]$, the expectation of our distribution; a ranking is correct if it provides higher variable importance for all used variables than it does for all unused variables.
%We use the ordering of these values as the variable importance ranking for \ourvi. 

We compare the rankings produced by $\ourvi$ with baseline methods, whose details are provided in the appendix: $\phi^{\text{sub}}$ to a random forest \citep{breiman2001random}; $\phi^{\text{sub}}$ to a L1 regularized logistic regression model; conditional model reliance, as defined in \cite{FisherRuDo19}, applied to a random forest (which is designed to capture only unique information of a variable); conditional model reliance applied to a L1 regularized logistic regression model; the impurity based measure of model reliance for random forests proposed in \cite{breiman2001statistical}; the LOCO algorithm reliance \cite{lei2018distribution} value for random forests; the LOCO algorithm reliance \cite{lei2018distribution} value for L1 regularized logistic regression; the Pearson and Spearman correlation between each feature and the outcome; the mean of the partial dependency plot \citep{greenwell2018simple} for each feature;  the SHAP \cite{lundberg2018consistent} value for each feature for a random forest; and, finally, we compute rankings from the mean VIC \cite{dong2020exploring} value for the Rashomon set of sparse decision trees. 
In order to support fair comparison, we evaluate each baseline variable importance method for each variable across $500$ bootstrap samples and compute the mean of these values, with the exception of VIC, for which we simply take the average VI value across the Rashomon set for the original dataset because VIC already calculates a range of values. 

Figure \ref{fig:baseline-rankings} reports the proportion of variables that are ranked in accordance with the ground truth for each dataset and each variable importance metric.
%We use the ordering of these values as the variable importance ranking given by each baseline method. Finally, we evaluate what proportion of variables are ranked in accordance with the ground truth for each dataset and each variable importance metric. These proportions are summarized in Figure \ref{fig:baseline-rankings}.
As shown in Figure \ref{fig:baseline-rankings}, $\ourvi$ correctly recovers the rankings of all variables in each dataset. Four baseline methods --- model reliance applied to random forests, permutation importance for random forests, VIC, and impurity based importance for random forests --- achieve the same result. All other baseline models have higher rates of disagreement with the ground truth ranking on at least one dataset. Motivated by this finding, we next explore how well each subtractive model reliance based method recovers the true value for subtractive model reliance on the DGP, allowing us to distinguish between the best performing models in Figure \ref{fig:baseline-rankings}. %VIC achieves low levels of agreement with both versions of the Hooker dataset at 60\% agreement with each.

\subsection{Recovering the Value of a Variable Importance Measurement On the DGP}
\label{subsec:recovering-values}
\input{paper_files/coverage}
%\begin{figure*}[h!]
%    \centering
%     \includegraphics[width=\textwidth]{figures/baseline_distributions_tmp.png}
%    \caption{Subtractive model reliance distributions for Monk 1 and 3 datasets. The dotted line represents ground truth, namely the subtractive model reliance for the variable calculated using the DGP. MR LASSO and MR RF denote subtractive model reliance applied to a $\ell_1$ regularized logistic regression model and a random forest respectively.}
%    \label{fig:monk-distributuions}
%\end{figure*}
%\begin{table}[]
%    \centering
%    \begin{tabular}{c|c|c|c|c|c|c||c}
%        \hline
%        Method & $X_1$  & $X_2$  & $X_3$  & $X_4$  & $X_5$  & $X_6$  & Mean \\
%        %
%        %
%        \hline
%        \rowcolor{Gainsboro!60}
%        \multicolumn{8}{l}{Monk 1} \\\hline
%        VIC & 0.062 & 0.063  & 0.002 & 0.004 & 0.073 & 0.004 & \textbf{0.035}\\
%        MR Random Forest & 0.101 & 0.105 & 0.061 & 0.072 & 0.004 & 0.055 & 0.067\\
%        MR Lasso & 0.286 & 0.309 & 0.016  & 0.016 & 0.12 & 0.011 & 0.126\\
%        \ourvi & 0.068 & 0.082  & 0.008 & 0.011 & 0.074 & 0.011 &0.043\\
%        %
%        %
%        \hline
%        \rowcolor{Gainsboro!60}
%        \multicolumn{8}{l}{Monk 3} \\\hline
%        VIC & 0.001 & 0.022 & 0.005 & 0.025 & 0.058 & 0.000 & 0.018\\
%        MR Random Forest & 0.038 & 0.026 & 0.035 &0.009 & 0.006 & 0.022 & 0.023\\
%        MR Lasso & 0.009 & 0.095 & 0.008 & 0.026 & 0.098 & 0.027 & 0.044\\
%        \ourvi & 0.010 & 0.006 & 0.013 & 0.019 & 0.036 & 0.005 & \textbf{0.015}\\
%        %
%        %
%        \hline
%        \rowcolor{Gainsboro!60}
%        \multicolumn{8}{l}{Friedman's} \\\hline
%        VIC & 0.061 & 0.043 & 0.080 & 0.008 & 0.076 & & 0.053\\
%        MR Random Forest & 0.018 & 0.063 & 0.047 & 0.040 & 0.052 & & 0.044\\
%        MR Lasso & 0.011 & 0.099 & 0.077 & 0.047 & 0.037 & & 0.054\\
%        \ourvi & 0.037 & 0.039 & 0.065 & 0.020 & 0.056 & & \textbf{0.043}\\
%        
%    \end{tabular}
%    \caption{Earth movers distance between model reliance on the DGP and estimates. }
%    \label{tab:emd_table}
%\end{table}
%

%\begin{table}[]
%    \centering
%    \begin{tabular}{c|c|c|c|c|c|c|c||c}
%        \hline
%        Dataset & Method & $X_1$  & $X_2$  & $X_3$  & $X_4$  & $X_5$  & $X_6$  & Mean \\
%        %
%        %
%        \hline
%        \rowcolor{Gainsboro!60}
%        Monk 1 &\ourvi & 1.0 & 1.0 & 1.0  & 1.0 &1.0 & 1.0 & \textbf{1.0}\\
%        &MR AdaBoost & 0.0 & 0.0 & 1.0 & 1.0 & 0.948 & 1.0 & 0.658\\
%         &MR GOSDT & 1.0 & 1.0 & 1.0  & 1.0 & 1.0 & 1.0 & \textbf{1.0}\\
%         &MR Lasso & 0.0 & 0.0 & 1.0 & 1.0 & 0.870 & 1.0 & 0.645\\
%        &MR Random Forest & 0.496 & 0.452 & 1.0 & 1.0 & 1.0 & 1.0 & 0.825\\
%        & VIC & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & \textbf{1.0}\\
%        %
%        %
%        \hline
%        \rowcolor{Gainsboro!60}
%        Monk 3 &\ourvi & 1.0 & 1.0 & 1.0 & 1.0 & 0.994 & 1.0 & \textbf{0.999} \\
%        &MR AdaBoost & 1.0 & 1.0 & 1.0 & 1.0 & 0.962 & 1.0 & 0.994\\
%        &MR GOSDT & 1.0 & 1.0 & 1.0 & 0.0 & 0.996 & 1.0 & 0.833\\
%        &MR Lasso & 1.0 & 0.990 & 1.0 & 0.744 & 1.0 & 1.0 & 0.956\\
%        &MR Random Forest & 1.0 & 0.968 & 1.0 & 1.0 & 0.992 & 1.0 & 0.993 \\
%        & VIC & 1.0 & 0.772 & 1.0 & 0.926 & 0.052 & 1.0 & 0.792\\
%        %
%        %
%        \hline
%        \rowcolor{Gainsboro!60}
%        Friedman's & \ourvi & 1.0 & 1.0 & 0.638 & 1.0 & 0.960 & & 0.920\\
%        & MR AdaBoost & 0.99 & 0.928 & 1.0 & 1.0 & 0.986 && \textbf{0.981}\\
%        & MR GOSDT & 0.075 & 0.070 & 0.0 & 0.070 & 0.026 & & 0.048\\
%        & MR Lasso & 1.0 & 0.222 & 0.002 & 0.978 & 0.962 & & 0.633\\
%        & MR Random Forest &  0.996 & 0.914 & 0.512 & 0.984 & 0.300 && 0.741\\
%        & VIC & 0.996 & 0.778 & 0.338 & 1.0 & 0.424 & & 0.707 \\
%        \hline
%        %
%        %
%        %\hline
%        %\rowcolor{Gainsboro!60}
%        %\multicolumn{8}{l}{Hooker Synth} \\\hline
%        %MR AdaBoost & 0.026 & 0.006 & 0.0 & 0.014 & 0.004 & 1.0, 0.0, 0.0, 0.04, 0.3 & 0.139\\
%        %MR GOSDT & \\
%        %MR Lasso & 0.824 & 0.968 & 0.986 & 0.896 & 0.986 & 1.0, 0.998, 0.87, 0.834, 0.932 & \textbf{0.929}\\
%        %MR Random Forest & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.67, 0.0, 0.0, 0.0, 0.0 & 0.070\\
%        %VIC & \\
%        %\ourvi & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 &0.904, 0.0, 0.0, 0.0, 0.0 & 0.090
%        
%    \end{tabular}
%    \caption{Coverage of subtractive model reliance values for the DGP across independent samples of the dataset by the IQR.}
%    \label{tab:emd_table}
%\end{table}
%
We can evaluate any variable importance metric $\phi$ using the known DGP and assess the ability of $\ourvi$ and other methods to recover the variable importance for the DGP for a fixed metric $\phi$.
%Note that, even when evaluating the DGP as our model, the value of $\phi(DGP, \mathcal{D}^{(n)}, v)$ still depends on the random quantity $\mathcal{D}^{(n)}$. As such, we evaluate $\phi(DGP, \mathcal{D}^{(n)}, v)$ across $B=500$ bootstrap iterations and consider $\frac{1}{B}\sum_{b=1}^B\phi(DGP, \mathcal{D}^{(n)}, v)$ to be the ground truth variable importance value.
We evaluate $\phi$ on a random forest model and a LASSO linear regression model for each of $B=500$ bootstrap samples and consider the distribution of these values, and measure the earth mover's distance (EMD) between the resulting distribution and the distribution of model reliance on the DGP across datasets of size $n$. In order to further investigate the comparison between random forest model reliance and \ourvi from Figure \ref{fig:baseline-rankings}, we focus our experiments around the Monk datasets, which are well-modeled as sparse decision trees. 
%Because the Hooker datasets have linear data generating processes, sparse decision trees would require large depth bounds to model these data effectively; therefore, 
%We focus our experiments around the Monk datasets, which are well-modeled as sparse decision trees. 
% While it is no surprise that the Rashomon set of sparse decision trees can recover the \textit{relative} ranking of the Hooker data sets as it can learn which variables are important, it is unlikely that optimal sparse decision trees will find \textit{absolute} variable importance values that closely resemble a completely different DGP.

%Table \ref{tab:emd_table} shows the resulting EMD relative to ground truth for each variable over three synthetic datasets. As shown in Table \ref{tab:emd_table}, \ourvi provides a better approximation of the underlying data distribution than all other methods in two out of three datasets evaluated. \ourvi consistently achieves lower EMD to the ground truth distribution than model reliance applied to random forests or lasso, demonstrating that the Rashomon set generally captures the reasoning of the DGP better than a set of non-optimal models (i.e., random forest). 

%Figure \ref{fig:monk-distributuions} (top) shows the resulting distributions of model reliance for Monk 1. As the first two subplots indicate, the distributions of model reliance for both LASSO and random forest models do not capture the expected model reliance for the DGP on variables 1 and 2. In contrast, $\ourvi$ captures the expected model reliance for the DGP on \textit{all} variables, with \textit{the mass of the distribution centered at the target value.} Figure \ref{fig:monk-distributuions} (bottom) shows the distributions of model reliance for Monk 3. In this case, we see that $\ourvi$ again captures the target value for each variable, with high mass around the true value. We observe that, on Monk 3, the distribution of model reliances for LASSO models does not capture the true reliance on variable 4. Similarly, the distribution of model reliances for random forest models overestimates the importance of variable 3. Even though random forests already account for sampling bias because of their in-built bootstrap procedure, accounting for the Rashomon effect enables us to capture true variable importance more accurately.




%\subsection{Summary of Results on Simulated Data}
%As shown in Section \ref{subsec:recovering-rankings}, \ourvi captures the true ranking of variable importance more effectively than the majority of baseline models, and equally as effectively as the best performing baseline models. Section \ref{subsec:recovering-values} highlights that \ourvi more effectively captures the \textit{true value} of model reliance than prior methods. Unlike previous methods, \ourvi is able to accurately reflect the underlying data distribution in the case of both the Monk datasets \textit{and} the Hooker datasets. By leveraging the entire Rashomon set for sparse decision trees across many bootstrap datasets, \ourvi is able to overcome finite sample constraints; in doing so, we can now trust discoveries found using RID can generalize to the underlying data distribution. 



% \begin{table*}
%     \centering
%     \begin{tabular}{l|l|l|l|l|l|l|l|l|l|l|l|l|l}
% \hline
% dataset & CMR RF & CMR L & L & LOCO L & LOCO RF & MR L & MR RF & Ours & PDP & Pear & RF Imp & SHAP & Spear\\
% \hline
% Hooker $(\rho = 0.9)$ & $0.8$ & $\mathbf{1}$ & $\mathbf{1}$ & $0.6$ & $0.5$ & $\mathbf{1}$ & $0.8$ & $0.8$ & $0.2$ & $0.6$ & $0.8$ & $0.4$ & $0.6$\\
% \hline
% Hooker $(\rho = 0)$ & $\mathbf{1}$ & $\mathbf{1}$ & $\mathbf{1}$ & $\mathbf{1}$ & $0.5$ & $\mathbf{1}$ & $\mathbf{1}$ & $\mathbf{1}$ & $0.4$ & $0.8$ & $\mathbf{1}$ & $0.5$ & $0.8$\\
% \hline
% Monk 1 & $\mathbf{1}$ & $0.83$ & $0.33$ & $0.67$ & $\mathbf{1}$ & $0.33$ & $\mathbf{1}$ & $\mathbf{1}$ & $0.33$ & $0.67$ & $\mathbf{1}$ & $\mathbf{1}$ & $0.67$\\
% \hline
% Monk 3 & $0.67$ & $0.67$ & $0.67$ & $0.67$ & $0.67$ & $0.67$ & $\mathbf{1}$ & $\mathbf{1}$ & $0.33$ & $0.67$ & $\mathbf{1}$ & $0.67$ & $0.67$\\
% \hline
% \end{tabular}
%     \caption{Caption}
%     \label{tab:my_label}
% \end{table*}

==> paper_files/synthetic_experiments_old.tex <==
In this section, we validate \ourvi using datasets with known data generating processes (DGP's). Since there is no universally accepted method for measuring the importance of a given variable to a model, we first evaluate \ourvi{}'s ability to recover the \textit{ranking} of variable importances for the DGP across several datasets with natural definitions for the ground truth variable importance rankings in \ref{subsec:recovering-rankings}. Evaluating our ability to recover rankings enables us to evaluate the accuracy of a given variable importance method without subscribing to a specific metric $\phi$.
In \ref{subsec:recovering-values} we evaluate $\phi$ on a known DGP for a fixed metric $\phi$ and measure the ability of \ourvi to recover the value of $\phi$ as applied to the DGP. In doing so, we evaluate the \ourvi's ability to capture the variable importance for the DGP under a fixed metric.

In both cases, we consider four datasets: Monk 1 and Monk3 \cite{thrun1991monk}, which each follow a distinct non-linear DGP; and the linear DGP described in \cite{hooker2021unrestricted} both with and without correlation between variables referred to as ``Hooker $(\rho = 0.9)$'' and ``Hooker $(\rho = 0)$'' respectively.\footnote{We exclude Monk 2 from our experiments because there is no clear notion of an expected variable importance ranking for this dataset, since the DGP involves all variables.} We convert the the datasets described in \cite{hooker2021unrestricted} into binary classification tasks by setting our label to $1$ if and only if the original outcome is greater than the median. See the Appendix for a more detailed description of the experimental setup.

%\begin{table}[h!]
%    \centering
%    \begin{tabular}{c|c|c}
%        Dataset & Features & DGP  \\
%        \hline
%        Monk 1 & 6 & ($a_1$ = $a_2$) or ($a_5$ = 1)\\
%        Monk 2 & 6 & EXACTLY TWO of:
%        \\&&\{$a_1$ = 1, $a_2$ = 1, 
%        \\&&$a_3$ = 1, $a_4$ = 1,
%        \\&&$a_5$ = 1, $a_6$ = 1\}\\
%        Monk 3 & 6 & (a5 = 3 and a4 = 1) 
%        \\&&or (a5 $\neq$ 4 and a2 $\neq$ 3)\\
%        Hooker & 10 & $a_1 + a_2 + a_3 + a_4$\\
%        &&$ + a_5 + 0a_6 + 0.5a_7$
%        \\&&$ + 0.8a_8 + 1.2a_9 + 1.5a_{10}$
%    \end{tabular}
%    \caption{Overview of the DGP used in our example datasets. In the Monk datasets, $a_1, \ldots, a_6$ take on values $\{1, 2, 3, 4\}$. In the Hooker datasets, $a_1, \ldots, a_{10}$ take on real values between 0 and 1.}
%    \label{tab:dgps}
%\end{table}

Throughout the following sections, we evaluate \ourvi using the Rashomon set of sparse decision trees as extracted by the TreeFARMS algorithm of \cite{xin2022exploring}. For all of our experiments except for those on the Hooker dataset with $\rho=0.9$, we evaluate \ourvi using subtractive model reliance $\phi_{\text{sub}}$ \citep{FisherRuDo19}, defined as
\begin{align}
    \label{eq:sub-mr}
    \phi_{\text{sub}}(f, \mathcal{D}^{(n)}, v) &= \ell_{\text{switch}} - \ell(f, \mathcal{D}^{(n)}),
\end{align}
where $\ell$ is $0-1$ misclassification loss function, $\ell_{\text{switch}}$ is defined as
\begin{align*}
    \ell_{\text{switch}} &= 
    \frac{1}{|P(\mathcal{D}^{(n)}, v)|}\sum_{\mathcal{D}_{\text{perm}}^{(n)} \in \mathcal{P}^{(v)}_{\mathcal{D}^{(n)}}} \ell(f, \mathcal{D}_{\text{perm}}^{(n)}),
\end{align*}
and $\mathcal{P}^{(v)}_{\mathcal{D}^{(n)}}$ denotes the set of datasets for all permutations of $X_1^{(v)}, X_2^{(v)}, \hdots, X_n^{(v)}$. For computational efficiency, we estimate $\ell_{\text{switch}}$ using the $e_{\text{divide}}$ strategy recommended in \cite{FisherRuDo19}. The metric $\phi_{\text{sub}}$ captures how much worse a model performs when the information given by $X^{(v)}$ is scrambled. In the case of the Hooker dataset with high correlation, we evaluate $\ourvi$ using the conditional model reliance (CMR) metric proposed in \cite{FisherRuDo19} over the 0-1 misclassification loss function. CMR is designed to capture the \textit{unique} information offered by a variable, and as such is expected to perform better in the presence of highly correlated variables.


\subsection{Recovering Rankings}
\label{subsec:recovering-rankings}

\begin{figure*}[ht]
    \centering
    % \includegraphics[width=0.98\linewidth]{figures/baseline_rankings.png}
    
    % \include{figures/baseline_rankings_tikz.tex}
    \caption{The proportion of features ranked correctly by each baseline model on each data set. RF indicates a random forest model, and lasso indicates a L1 regularized logistic regression model. PDP indicates partial dependency plots, CMR indicates conditional model reliance, and all other acronyms are defined as elsewhere in the paper.}
    \label{fig:baseline-rankings}
\end{figure*}

The ground truth variable importance ranking is uniquely defined for each dataset we consider. For Monk 1 and Monk 3, we define variable importance based on whether a given variable appears in the DGP or not. For the linear datasets proposed in \cite{hooker2021unrestricted}, we define the ground truth variable importance ranking based on the coefficient on each variable. 
%=\{ \{(X_i^{(j)}, X_i^{(v)}, Y_i)\}_{i=1}^n \}$
We extract variable importance rankings from \ourvi by evaluating \ourvi for each variable in a given dataset $\mathcal{D}^{(n)}$ across $B=500$ bootstrap samples and estimating $\mathbb{E}[\ourvi]$, the expectation of our distribution. 
We use the ordering of these values as the variable importance ranking for \ourvi. 

We compare the rankings produced by \ourvi with those produced by the following baseline methods: $\phi_{\text{sub}}$ to a random forest \cite{breiman2001random}; $\phi_{\text{sub}}$ to a L1 regularized logistic regression model; conditional model reliance, as defined in \cite{FisherRuDo19}, applied to a random forest; conditional model reliance applied to a L1 regularized logistic regression model; the impurity based measure of model reliance for random forests proposed in \cite{breiman2001statistical}; the LOCO algorithm reliance \cite{lei2018distribution} value for random forests; the LOCO algorithm reliance \cite{lei2018distribution} value for L1 regularized logistic regression; the Pearson and Spearman correlation between each feature and the outcome; the mean of the partial dependency plot \citep{greenwell2018simple} for each feature;  the SHAP \cite{lundberg2018consistent} value for each feature for a random forest; and, finally, we compute rankings from the mean VIC \cite{dong2020exploring} value for the Rashomon set of sparse decision trees. 

In order to support fair comparison, we evaluate each baseline variable importance method for each variable across $500$ bootstrap samples and compute the mean of these values, with the exception of VIC, for which we simply take the average VI value across the Rashomon set for the original dataset because VIC already calculates a range of values. We use the ordering of these values as the variable importance ranking given by each baseline method. Finally, we evaluate what proportion of variables are ranked in accordance with the ground truth for each dataset and each variable importance metric. These proportions are summarized in Figure \ref{fig:baseline-rankings}.

As shown in Figure \ref{fig:baseline-rankings}, \ourvi correctly recovers the rankings of all variables in each dataset except for the Hooker dataset with highly correlated variables. On this dataset, \ourvi recovers the correct ranking for 80\% of variables. Two baseline methods --- model reliance applied to random forests and impurity based importance for random forests --- achieve the same result. All other baseline models except VIC have higher rates of disagreement with the ground truth ranking on the Monk 3 dataset, and most baseline models achieve similar rates of agreement on the Hooker dataset with $\rho=0.9$. VIC achieves low levels of agreement with both versions of the Hooker dataset at 60\% agreement with each.


\subsection{Recovering the Value of a Metric Over the DGP}
\label{subsec:recovering-values}
\begin{figure*}[h!]
    \centering
     \include{figures/monk1_distributions.tex}
    \caption{Subtractive model reliance distributions for Monk 1 and 3 datasets. The dotted line represents the subtractive model reliance for the variable calculated using the DGP. MR Lasso and MR RF denote subtractive model reliance applied to a L1 regularized logistic regression model and a random forest respectively.}
    \label{fig:monk-distributuions}
\end{figure*}

Although the importance of a variable to the DGP is not well defined in general, we can evaluate any variable importance metric $\phi$ using the known DGP as our model. This provides a numerical baseline that any method using the metric $\phi$ should aim to replicate. In this section, we evaluate the ability of \ourvi to recover the variable importance for the DGP for a fixed metric $\phi$. Note that, even when evaluating the DGP as our model, the value of $\phi(DGP, \mathcal{D}^{(n)}, v)$ still depends on the random quantity $\mathcal{D}^{(n)}$. As such, we evaluate $\phi(DGP, \mathcal{D}^{(n)}, v)$ across $B=500$ bootstrap iterations and consider $\frac{1}{B}\sum_{b=1}^B\phi(DGP, \mathcal{D}^{(n)}, v)$ to be the ground truth variable importance value.

We evaluate $\phi$ on a random forest model and a lasso linear regression model for each of $B=500$ bootstrap samples and consider the distribution of these values across bootstrap iterations for comparison. Because the Hooker datasets have linear data generating processes, sparse decision trees would require large depth bounds to model these data effectively; therefore, we focus our experiments around the Monk datasets, which would likely be well-modeled as sparse decision trees. 
% While it is no surprise that the Rashomon set of sparse decision trees can recover the \textit{relative} ranking of the Hooker data sets as it can learn which variables are important, it is unlikely that optimal sparse decision trees will find \textit{absolute} variable importance values that closely resemble a completely different DGP.

Figure \ref{fig:monk-distributuions} (top) shows the resulting distributions of model reliance for Monk 1. As the first two subplots indicate, the distributions of model reliance for both lasso and random forest models do not capture the expected model reliance for the DGP on variables 1 and 2. In contrast, $\ourvi$ captures the expected model reliance for the DGP on \textit{all} variables, with \textit{the mass of the distribution centered at the target value.}

Figure \ref{fig:monk-distributuions} (bottom) shows the resulting distributions of model reliance for Monk 3. In this case, we see that $\ourvi$ again captures the target value for each variable, with high mass around the true value. We observe that, on Monk 3, the distribution of model reliances for Lasso models does not capture the true reliance on variable 4. Similarly, the distribution of model reliances for random forest models overestimates the importance of variable 3. Even though random forests can model the Monk datasets well and already account for sampling bias because of their in-built bootstrap procedure, accounting for the Rashomon effect enables us to capture true variable importance more accurately.

\subsection{Summary of Results on Simulated Data}
As shown in Section \ref{subsec:recovering-rankings}, \ourvi captures the true ranking of variable importance more effectively than the majority of baseline models, and equally as effectively as the best performing baseline models. Section \ref{subsec:recovering-values} highlights that \ourvi more effectively captures the \textit{true value} of model reliance than prior methods. Unlike previous methods, \ourvi is able to accurately reflect the underlying data distribution in the case of both the Monk datasets \textit{and} the Hooker datasets. By leveraging the entire Rashomon set for sparse decision trees across many bootstrap datasets, \ourvi is able to overcome finite sample constraints; in doing so, we can now trust discoveries found using RID can generalize to the underlying data distribution. 



% \begin{table*}
%     \centering
%     \begin{tabular}{l|l|l|l|l|l|l|l|l|l|l|l|l|l}
% \hline
% dataset & CMR RF & CMR L & L & LOCO L & LOCO RF & MR L & MR RF & Ours & PDP & Pear & RF Imp & SHAP & Spear\\
% \hline
% Hooker $(\rho = 0.9)$ & $0.8$ & $\mathbf{1}$ & $\mathbf{1}$ & $0.6$ & $0.5$ & $\mathbf{1}$ & $0.8$ & $0.8$ & $0.2$ & $0.6$ & $0.8$ & $0.4$ & $0.6$\\
% \hline
% Hooker $(\rho = 0)$ & $\mathbf{1}$ & $\mathbf{1}$ & $\mathbf{1}$ & $\mathbf{1}$ & $0.5$ & $\mathbf{1}$ & $\mathbf{1}$ & $\mathbf{1}$ & $0.4$ & $0.8$ & $\mathbf{1}$ & $0.5$ & $0.8$\\
% \hline
% Monk 1 & $\mathbf{1}$ & $0.83$ & $0.33$ & $0.67$ & $\mathbf{1}$ & $0.33$ & $\mathbf{1}$ & $\mathbf{1}$ & $0.33$ & $0.67$ & $\mathbf{1}$ & $\mathbf{1}$ & $0.67$\\
% \hline
% Monk 3 & $0.67$ & $0.67$ & $0.67$ & $0.67$ & $0.67$ & $0.67$ & $\mathbf{1}$ & $\mathbf{1}$ & $0.33$ & $0.67$ & $\mathbf{1}$ & $0.67$ & $0.67$\\
% \hline
% \end{tabular}
%     \caption{Caption}
%     \label{tab:my_label}
% \end{table*}

==> supplement_files/ecr_ccr_proof.tex <==
%%% NOT READY FOR REVIEW 

\begin{corollary}
    % Let $\varepsilon_H, \delta > 0$. 
    The $\alpha$-central credible region ($CCR$) describes the range of values in  which $100\cdot(1-\alpha)\%$ of a distribution's central mass lies. In a univariate distribution, this quantity can be found using the $\frac{\alpha}{2}$ and $(1 - \frac{\alpha}{2})$ quantiles. The $\tau$-th quantile of a random variable $A$ is any value of $k$ such that $\mathbb{P}(A \leq k) = \tau.$ We define a new robustness region, the estimated coverage region ($ECR$): given $\varepsilon_E > 0,$ let $\tau_{low} = \frac{\alpha}{2} - 2\varepsilon_E$ and $\tau_{up} = 1 - \frac{\alpha}{2} + 2\varepsilon_E.$ Then, define 
    \begin{align*}
        ECR = \left(\hat{Q}_{\tau_{low}}, \hat{Q}_{\tau_{up}} \right),
    \end{align*}
    where $Q_{\widehat{\ourvi}}(\tau)$ is the $\tau$-th quantile of $\widehat{\ourvi}$.
    
    With high probability, $ECR$ is guaranteed to cover $\ourvi's$ $CCR$ using $\widehat{\ourvi}$. Specifically, with probability $1 - \delta,$
    \begin{align*}
        CCR \subset ECR
    \end{align*}
    with $B \geq \frac{1}{2\varepsilon^2}\ln\left( \frac{8}{\delta} \right)$ bootstrap iterations.
    
    % Let $Q_{\frac{\alpha/2}}$ and $Q_{1 - \frac{\alpha}{2}}$ represent the $\alpha\%-$central credible region in $\ourvi.$ These are the $\frac{\alpha}{2}$ and $100 - \frac{\alpha}{2}$ percentiles in $\ourvi.$ 
    
    % Given quantiles of interest $t_{\text{low}}$ and $t_{\text{up}}$ such that $t_{\text{low}} < t_{\text{up}}$, let $\tau_{\text{low}}:= t_{\text{low}} - 2\varepsilon_H $ and $\tau_{\text{up}}:= t_{\text{up}} + 2\varepsilon_H $. Let $CCR(t_{\text{low}}, t_{\text{high}}):=\mathbb{P}(\ourvi \leq Q_{\ourvi}(t_{\text{low}}) ), \mathbb{P}(\ourvi \leq Q_{\ourvi}(t_{\text{up}}) )$ denote the region between the $t_{\text{low}}$-th quantile and the $t_{\text{up}}$-th quantile of $\ourvi$, and let $\widehat{CCR}(\tau_{\text{low}}, \tau_{\text{up}}):=\mathbb{P}(\widehat{\ourvi} \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) ), \mathbb{P}(\widehat{\ourvi} \leq Q_{\widehat{\ourvi}}(t_{\text{up}}) )$ denote the region between the $\tau_{\text{low}}$-th quantile and the $\tau_{\text{up}}$-th quantile of $\widehat{\ourvi}$.
%     Then, with probability at least $1 - 4\delta$,
%     \begin{align*}
%         \left(\mathbb{P}(\ourvi \leq Q_{\ourvi}(t_{\text{low}}) ), \mathbb{P}(\ourvi \leq Q_{\ourvi}(t_{\text{up}}) )\right)\subseteq \left(\mathbb{P}(\widehat{\ourvi} \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) ), \mathbb{P}(\widehat{\ourvi} \leq Q_{\widehat{\ourvi}}(\tau_{\text{up}}) )\right)
%     \end{align*}
% with $B \geq \frac{\ln\left( \frac{1 - \delta}{2} \right)}{-2\varepsilon_H^2}$ iterations.
\end{corollary}
\begin{proof}
%     Let $\alpha \in (0, 1), \varepsilon_H > 0, \delta > 0.$ Let $\hat{Q}_\tau$ denote the $\tau$-th quantile of $\widehat{\ourvi}$ and $Q_\tau$ denote the $\tau$-th quantile of $\ourvi,$ i.e. $Q_\tau$ is the value of $k$ such that $\mathbb{P}(\ourvi \leq k) = \tau.$ Let $\tau_{low} = \min\left\{0, \frac{\alpha}{2} - 2\varepsilon_H\right\}$ and $\tau_{up} = \max\left\{0, \frac{\alpha}{2} + 2\varepsilon_H\right\}.$ Assume we run $B \geq \frac{1}{2\varepsilon_H^2}\ln\left( \frac{2}{\delta} \right)$ bootstrap iterations. By Theorem \ref{thm:ourvi_finite_sample}, the following holds:
%     \begin{align*}
%         \mathbb{P}\left(\left| \mathbb{P}(\widehat{\ourvi} \leq k ) - \mathbb{P}(\ourvi \leq k )\right| \leq \varepsilon_H \right) \geq 1 -\delta,
%     \end{align*}
%     which implies
%     \begin{align*}
%         &\mathbb{P}\left( \mathbb{P}(\ourvi \leq k ) - \mathbb{P}(\widehat{\ourvi} \leq k ) \leq \varepsilon_H  \right) \geq 1 - \delta \text{ and } \mathbb{P}\left( \mathbb{P}(\widehat{\ourvi} \leq k )  - \mathbb{P}(\ourvi \leq k )\leq \varepsilon_H  \right) \geq 1 -\delta.
%     \end{align*}

%     Because this result holds for any $k \in [\phi_{min}, \phi_{max}],$ this result also holds for $\hat{Q}_{\tau_{low}}:$
%     \begin{align*}
%         &\mathbb{P}\left( \mathbb{P}(\ourvi \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) ) - \mathbb{P}(\widehat{\ourvi} \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) ) \leq \varepsilon_H  \right) \geq 1 -\delta.
%     \end{align*}
%     Because $\mathbb{P}\left(\widehat{RID} \leq \hat{Q}_{\tau_{low}} \right) = \frac{\alpha}{2} - 2\varepsilon_H,$ we know that
%     \begin{align*}
%         &\mathbb{P}\left( \mathbb{P}(\ourvi \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) ) - \mathbb{P}(\widehat{\ourvi} \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) ) \leq \varepsilon_H  \right) \\
% =  &\mathbb{P}\left( \mathbb{P}(\ourvi \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) ) \leq \varepsilon_H + \mathbb{P}(\widehat{\ourvi} \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) )  \right) \\
% = &\mathbb{P}\left( \mathbb{P}(\ourvi \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) ) \leq \varepsilon_H + \frac{\alpha}{2} - 2\varepsilon_H \right) \\
% = &\mathbb{P}\left( \mathbb{P}(\ourvi \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) ) \leq \frac{\alpha}{2} - \varepsilon_H \right).
%     \end{align*}

% Because $\mathbb{P}\left( \mathbb{P}(\ourvi \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) ) - \mathbb{P}(\widehat{\ourvi} \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) ) \leq \varepsilon_H  \right) \geq 1 -\delta,$ we know that
% \begin{align*}
%     &\mathbb{P}\left( \mathbb{P}(\ourvi \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) ) - \mathbb{P}(\widehat{\ourvi} \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) ) \geq \varepsilon_H  \right) \\
%     = & 1 - \mathbb{P}\left( \mathbb{P}(\ourvi \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) ) - \mathbb{P}(\widehat{\ourvi} \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) ) \leq \varepsilon_H  \right) \\
%     \geq & 1 - \delta.
% \end{align*}
% Therefore, 
% \begin{align*}
%     \mathbb{P}\left( \mathbb{P}(\ourvi \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) ) - \mathbb{P}(\widehat{\ourvi} \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) ) \leq \varepsilon_H  \right) &= 1 - \mathbb{P}\left( \mathbb{P}(\ourvi \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) ) - \mathbb{P}(\widehat{\ourvi} \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) ) > \varepsilon_H  \right) \leq \delta.
% \end{align*}

    % and
    % \begin{align*}
    %     &\mathbb{P}\left( \mathbb{P}(\widehat{\ourvi} \leq k )  - \mathbb{P}(\ourvi \leq k )\leq \varepsilon_H  \right) \geq 1 -\delta.
    % \end{align*}
    
    Let $t_{\text{low}}, t_{\text{up}} \in (0, 1)$ such that $t_{\text{low}} < t_{\text{up}}$, and let $\varepsilon_H, \delta > 0$. Let $Q_{\widehat{\ourvi}}(\tau)$ denote the $\tau$-th quantile of $\widehat{\ourvi}$ and $Q_{\ourvi}(\tau)$ denote the $\tau$-th quantile of $\ourvi$, that is, $\mathbb{P}(\widehat{\ourvi} \leq Q_{\widehat{\ourvi}}(\tau) ) = \tau$ and $\mathbb{P}(\ourvi \leq Q_{\ourvi}(\tau) ) = \tau$. Finally, let $\tau_{\text{low}} := t_{\text{low}} - 2\varepsilon_H$ and $\tau_{\text{up}} := t_{\text{up}} + 2\varepsilon_H$. Theorem \ref{thm:rid_finite_sample} states that, with $B \geq \frac{1}{2\varepsilon_H^2}\ln\left( \frac{2}{\delta} \right)$ bootstrap iterations, the following holds:
    \begin{align*}
        \mathbb{P}\left(\left| \mathbb{P}(\widehat{\ourvi} \leq k ) - \mathbb{P}(\ourvi \leq k )\right| \leq \varepsilon_H \right) \geq 1 -\delta,
    \end{align*}
    which implies the following looser bounds:
    \begin{align}
        &\mathbb{P}\left( \mathbb{P}(\ourvi \leq k ) - \mathbb{P}(\widehat{\ourvi} \leq k ) \leq \varepsilon_H  \right) \geq 1 -\delta
    \label{eq:rid-sub-est}
    \end{align}
    and
    \begin{align}
        &\mathbb{P}\left( \mathbb{P}(\widehat{\ourvi} \leq k )  - \mathbb{P}(\ourvi \leq k )\leq \varepsilon_H  \right) \geq 1 -\delta.
    \label{eq:est-sub-rid}
    \end{align}
    By Equation (\ref{eq:rid-sub-est}), we know that the probability of the following event is at least $1-\delta$:
    \begin{align*}
        & \mathbb{P}(\ourvi \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) ) - \mathbb{P}\left(\widehat{\ourvi} \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) \right) \leq \varepsilon_H  &\text{by setting $k = Q_{\widehat{\ourvi}}(\tau_{low})$}\\
        %
        & \iff  \mathbb{P}\left[\ourvi \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) \right] \leq \varepsilon_H + \mathbb{P}\left[\widehat{\ourvi} \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) \right] \\
        %
        & \iff \mathbb{P}\left[\ourvi \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) \right] \leq \varepsilon_H + t_{\text{low}} - 2 \varepsilon_H  &\text{ b.c. $\mathbb{P}[\widehat{\ourvi} \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}})] = t_{\text{low}} - 2 \varepsilon_H $ by definition}\\
        %
        & \iff \mathbb{P}\left[\ourvi \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) \right] \leq t_{\text{low}} - \varepsilon_H\\
    \end{align*}
    This states that, with high probability, the $\tau_{\text{low}}$ quantile of the distribution of $\widehat{\ourvi}$ is below the $t_{\text{low}} - \varepsilon_H$ quantile of $\ourvi$. We would like to explicitly draw a connection between some quantile of $\ourvi$ and $\widehat{\ourvi}$. To do so, we can then find the probability of the converse of the above as:
    \begin{align*}
        %
        &\mathbb{P}\left[\mathbb{P}\left(\ourvi \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) \right) \leq t_{\text{low}} - \varepsilon_H\right] \geq 1 - \delta \\
        %
        & \iff 1 - \mathbb{P}\left[ \mathbb{P}\left(\ourvi \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) \right) \leq t_{\text{low}} - \varepsilon_H\right] \leq \delta\\
        %
        & \iff \mathbb{P}\left[ \mathbb{P}\left(\ourvi \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) \right) > t_{\text{low}} - \varepsilon_H\right] \leq \delta\\
        %
        & \iff \mathbb{P}\left[ \mathbb{P}\left(\ourvi \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) \right) >  \mathbb{P}\left(\ourvi \leq Q_{\ourvi}(t_{\text{low}}) \right) - \varepsilon_H\right] \leq \delta &\text{ $t_{\text{low}} = \mathbb{P}\left(\ourvi \leq Q_{\ourvi}(t_{\text{low}})\right)$ by definition}\\
    \end{align*}
    %In other words, $Q_{\ourvi}(t_{\text{low}})$ is likely no more than $\varepsilon_H$ below $Q_{\widehat{\ourvi}}(\tau_{\text{low}})$. 
    
    We now use the above result to draw a connection between the (unknown) quantity $\mathbb{P}(\ourvi \leq Q_{\ourvi}(t_{\text{low}}) )$ and the (known) quantity $\mathbb{P}(\widehat{\ourvi} \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) )$ by reintroducing the converse of Equation (\ref{eq:est-sub-rid}). From above,
    \begin{align*}
        &  \mathbb{P}\left[ \mathbb{P}\left(\ourvi \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) \right) > \mathbb{P}\left(\ourvi \leq Q_{\ourvi}(t_{\text{low}}) \right) - \varepsilon_H\right] \leq \delta\\\\
        %
        \iff &\mathbb{P}\left[ \mathbb{P}\left(\ourvi \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) \right) >  \mathbb{P}\left(\ourvi \leq Q_{\ourvi}(t_{\text{low}}) \right) - \varepsilon_H\right] \\
        &+
        \mathbb{P}\left[\mathbb{P}\left(\widehat{\ourvi} \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) \right) - \mathbb{P}\left(\ourvi \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}})\right) \geq \varepsilon_H  \right]
        \leq \delta + \delta 
        &\text{By Equation (\ref{eq:est-sub-rid})}\\ \\
        %
        \iff &\mathbb{P}\left[ \underbrace{\varepsilon_H + \mathbb{P}(\ourvi \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) ) >  \mathbb{P}(\ourvi \leq Q_{\ourvi}(t_{\text{low}}) )}_{X} \right] \\
        &+
        \mathbb{P}\left[\underbrace{\mathbb{P}(\widehat{\ourvi} \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) ) \geq \varepsilon_H + \mathbb{P}(\ourvi \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}))}_{Y} \right]
        \leq 2 \delta\\\\
        %
        \implies &\mathbb{P}\Bigg[\left\{ \varepsilon_H + \mathbb{P}(\ourvi \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) ) >  \mathbb{P}(\ourvi \leq Q_{\ourvi}(t_{\text{low}}) ) \right\} \\
        &\cup
        \left\{\mathbb{P}(\widehat{\ourvi} \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) ) \geq \varepsilon_H + \mathbb{P}(\ourvi \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}))  \right\}\Bigg]
        \leq 2 \delta 
        &\text{By the Union Bound; since } \\
        &&\mathbb{P}(X \cup Y) \leq \mathbb{P}(X) + \mathbb{P}(Y) \leq 2\delta.
    \end{align*}
    This states that either (1) there is a small probability that $Q_{\widehat{\ourvi}}(\tau_{\text{low}})$ is larger than $Q_{\ourvi}(\tau_{\text{low}})$ or (2) there is a small probability that our estimate for $\ourvi$ at $Q_{\widehat{\ourvi}}(\tau_{\text{low}})$ is too large. We now invert this probability to show that, with high probability, $\mathbb{P}(\widehat{\ourvi} \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) )$ provides a lower bound on $ \mathbb{P}(\ourvi \leq Q_{\ourvi}(t_{\text{low}}) ) $:
    \begin{align*}
        %
        &\mathbb{P}\bigg[\left\{ \varepsilon_H + \mathbb{P}(\ourvi \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) ) >  \mathbb{P}(\ourvi \leq Q_{\ourvi}(t_{\text{low}}) ) \right\} \\
        &\cup
        \left\{\mathbb{P}(\widehat{\ourvi} \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) ) \geq \varepsilon_H + \mathbb{P}(\ourvi \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}))  \right\}\bigg]
        \leq 2 \delta\\
        \iff  & 1 - \mathbb{P}\bigg[\left\{ \varepsilon_H + \mathbb{P}(\ourvi \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) ) > \mathbb{P}(\ourvi \leq Q_{\ourvi}(t_{\text{low}}) ) \right\} \\
        &\cup
        \left\{\mathbb{P}(\widehat{\ourvi} \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) ) \geq \varepsilon_H + \mathbb{P}(\ourvi \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}))  \right\}\bigg]
        \geq 1 - 2 \delta\\
        %
        \iff & \mathbb{P}\bigg[\left\{ \varepsilon_H + \mathbb{P}(\ourvi \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) ) \leq \mathbb{P}(\ourvi \leq Q_{\ourvi}(t_{\text{low}}) ) \right\} \\
        &\cap
        \left\{\mathbb{P}(\widehat{\ourvi} \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) ) < \varepsilon_H + \mathbb{P}(\ourvi \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}))  \right\}\bigg]
        \geq 1 - 2 \delta
        \end{align*}
    Since the term $\varepsilon_H + \mathbb{P}(\ourvi \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}))$ appears in both of the interior inequalities above, we can simplify the intersection by combining the two inequalities:
        \begin{align*}
        \mathbb{P}\bigg[&\left\{ \varepsilon_H + \mathbb{P}(\ourvi \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) ) \leq \mathbb{P}(\ourvi \leq Q_{\ourvi}(t_{\text{low}}) ) \right\} \\
        &\cap
        \left\{\mathbb{P}(\widehat{\ourvi} \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) ) < \varepsilon_H + \mathbb{P}(\ourvi \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}))  \right\}\bigg]
        \geq 1 - 2 \delta\\
        %
        \iff & \mathbb{P}\left(\mathbb{P}(\widehat{\ourvi} \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) ) < \varepsilon_H + \mathbb{P}(\ourvi \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) ) \leq \mathbb{P}(\ourvi \leq Q_{\ourvi}(t_{\text{low}}) ) \right)
        \geq 1 - 2 \delta\\
        %
        \iff & \mathbb{P}\left(\mathbb{P}(\widehat{\ourvi} \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) ) < \mathbb{P}(\ourvi \leq Q_{\ourvi}(t_{\text{low}}) ) \right)
        \geq 1 - 2 \delta\\
        \iff & \mathbb{P}\left(\mathbb{P}(\widehat{\ourvi} \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) ) \geq \mathbb{P}(\ourvi \leq Q_{\ourvi}(t_{\text{low}}) ) \right)
        \leq 2 \delta
    \end{align*}
    
    In other words, it is likely that the $\tau_{\text{low}}$-th quantile of $\widehat{\ourvi}$ provides a lower bound on the $t_{\text{low}}$-th quantile of $\ourvi$. 
    
    By following the same structure, we can derive a similar upper bound on the $t_{\text{up}}$-th quantile of $\ourvi$ in terms of $\widehat{\ourvi}$, arriving at the following result:
    \begin{align*}
        \mathbb{P}\left(\mathbb{P}(\widehat{\ourvi} \leq Q_{\widehat{\ourvi}}(\tau_{\text{up}}) ) \leq \mathbb{P}(\ourvi \leq Q_{\ourvi}(t_{\text{up}}) ) \right)
        \leq 2 \delta
    \end{align*}



    
    
    %by leveraging Equation (\ref{eq:est-sub-rid}) as follows:
    %\begin{align*}
     %   &\mathbb{P}\left( \mathbb{P}(\widehat{\ourvi} \leq Q_{\widehat{\ourvi}}(\tau_{\text{up}}) ) - \mathbb{P}(\ourvi \leq Q_{\widehat{\ourvi}}(\tau) ) \leq \varepsilon_H  \right) \geq 1 -\delta\\
     %   \iff & \mathbb{P}\left( \mathbb{P}(\widehat{\ourvi} \leq Q_{\widehat{\ourvi}}(\tau_{\text{up}}) ) -  \varepsilon_H  \leq\mathbb{P}(\ourvi \leq Q_{\widehat{\ourvi}}(\tau) ) \right) \geq 1 -\delta\\
     %   \iff & \mathbb{P}\left( t_{\text{up}} + 2\varepsilon_H -  \varepsilon_H  \leq\mathbb{P}(\ourvi \leq Q_{\widehat{\ourvi}}(\tau_{\text{up}}) ) \right) \geq 1 -\delta 
        %
     %   &\text{ By definition of $Q_{\widehat{\ourvi}}(\tau_{\text{up}})$}\\
     %   \iff & \mathbb{P}\left( t_{\text{up}} + \varepsilon_H\leq\mathbb{P}(\ourvi \leq Q_{\widehat{\ourvi}}(\tau_{\text{up}}) ) \right) \geq 1 -\delta\\
     %   \iff & 1 - \mathbb{P}\left( t_{\text{up}} + \varepsilon_H \leq\mathbb{P}(\ourvi \leq Q_{\widehat{\ourvi}}(\tau_{\text{up}}) ) \right) \leq \delta\\
      %  \iff & \mathbb{P}\left(t_{\text{up}} + \varepsilon_H > \mathbb{P}(\ourvi \leq Q_{\widehat{\ourvi}}(\tau_{\text{up}})) \right) \leq \delta\\
        %
      %  \iff & \mathbb{P}\left(\mathbb{P}(\ourvi \leq Q_{\widehat{\ourvi}}(\tau_{\text{up}})) < t_{\text{up}} + \varepsilon_H\right) \leq \delta\\
        %
       % \iff & \mathbb{P}\left(\mathbb{P}(\ourvi \leq Q_{\widehat{\ourvi}}(\tau_{\text{up}})) - \varepsilon_H <  \mathbb{P}(\ourvi \leq Q_{\ourvi}(t_{\text{up}}) )  \right) \leq \delta
%\end{align*}
%As in the lower bound, we  draw a connection between the (unknown) quantity $\mathbb{P}(\ourvi \leq Q_{\ourvi}(t_{\text{up}}) )$ and the (known) quantity $\mathbb{P}(\widehat{\ourvi} \leq Q_{\widehat{\ourvi}}(\tau_{\text{up}}) )$ by reintroducing the converse of Equation (\ref{eq:rid-sub-est}):
%\begin{align*}
%        &\mathbb{P}\left(\mathbb{P}(\ourvi \leq Q_{\widehat{\ourvi}}(\tau_{\text{up}})) - \varepsilon_H <  \mathbb{P}(\ourvi \leq Q_{\ourvi}(t_{\text{up}}) )  \right) \leq \delta\\
%        \implies  &  \mathbb{P}\left(\mathbb{P}(\ourvi \leq Q_{\tau_{\text{up}}} ) - \mathbb{P}(\widehat{\ourvi} \leq Q_{\widehat{\ourvi}}(\tau_{\text{up}}) ) \geq  \varepsilon_H\right) \\
%        &+ 
%        \mathbb{P}\left( \mathbb{P}(\ourvi \leq Q_{\tau_{\text{up}}} ) - \varepsilon_H  < \mathbb{P}(\ourvi \leq Q_{\ourvi}(t_{\text{up}}) )   \right)
%        \leq 2 \delta \\
        %
 %       \iff   & \mathbb{P}\left(\mathbb{P}(\widehat{\ourvi} \leq Q_{\widehat{\ourvi}}(\tau_{\text{up}}) ) \leq \mathbb{P}(\ourvi \leq Q_{\tau_{\text{up}}} ) - \varepsilon_H\right) \\
%        &+ \mathbb{P}\left( \mathbb{P}(\ourvi \leq Q_{\tau_{\text{up}}} ) - \varepsilon_H  < \mathbb{P}(\ourvi \leq Q_{\ourvi}(t_{\text{up}}) )   \right)
%        \leq 2 \delta\\
%        \iff  &  \mathbb{P}\bigg(\left(\mathbb{P}(\widehat{\ourvi} \leq Q_{\widehat{\ourvi}}(\tau_{\text{up}}) ) \leq \mathbb{P}(\ourvi \leq Q_{\tau_{\text{up}}} ) - \varepsilon_H\right) \\
%        & \cup \left( \mathbb{P}(\ourvi \leq Q_{\tau_{\text{up}}} ) - \varepsilon_H  < \mathbb{P}(\ourvi \leq Q_{\ourvi}(t_{\text{up}}) )   \right)\bigg)
%        \leq 2 \delta\\
%        \iff  & 1 - \mathbb{P}\bigg(\left(\mathbb{P}(\widehat{\ourvi} \leq Q_{\widehat{\ourvi}}(\tau_{\text{up}}) ) \leq \mathbb{P}(\ourvi \leq Q_{\tau_{\text{up}}} ) - \varepsilon_H\right) \\
%        & \cup \left( \mathbb{P}(\ourvi \leq Q_{\tau_{\text{up}}} ) - \varepsilon_H  < \mathbb{P}(\ourvi \leq Q_{\ourvi}(t_{\text{up}}) )   \right)\bigg)
%        \geq 1 - 2 \delta\\
%        \iff  & \mathbb{P}\bigg(\left(\mathbb{P}(\widehat{\ourvi} \leq Q_{\widehat{\ourvi}}(\tau_{\text{up}}) ) > \mathbb{P}(\ourvi \leq Q_{\tau_{\text{up}}} ) - \varepsilon_H\right) \\
%        & \cap \left( \mathbb{P}(\ourvi \leq Q_{\tau_{\text{up}}} ) - \varepsilon_H  \geq \mathbb{P}(\ourvi \leq Q_{\ourvi}(t_{\text{up}}) )   \right)\bigg)
 %       \geq 1 - 2 \delta\\
 %       \iff  & \mathbb{P}\left(\mathbb{P}(\widehat{\ourvi} \leq Q_{\widehat{\ourvi}}(\tau_{\text{up}}) ) > \mathbb{P}(\ourvi \leq Q_{\tau_{\text{up}}} ) - \varepsilon_H  \geq \mathbb{P}(\ourvi \leq Q_{\ourvi}(t_{\text{up}}) )   \right)
 %       \geq 1 - 2 \delta\\
%        \implies  & \mathbb{P}\left(\mathbb{P}(\widehat{\ourvi} \leq Q_{\widehat{\ourvi}}(\tau_{\text{up}}) ) > \mathbb{P}(\ourvi \leq Q_{\ourvi}(t_{\text{up}}) ) \right)
 %       \geq 1 - 2 \delta\\
 %       \iff &  \mathbb{P}\left(\mathbb{P}(\widehat{\ourvi} \leq Q_{\widehat{\ourvi}}(\tau_{\text{up}}) ) \leq \mathbb{P}(\ourvi \leq Q_{\ourvi}(t_{\text{up}}) ) \right)
%        \leq 2 \delta
%    \end{align*}
%    In other words, $Q_{\ourvi}(t_{\text{up}})$ is likely bounded above by $Q_{\widehat{\ourvi}}(\tau_{\text{up}})$. 
    
    Finally, we can combine the upper and lower bounds we found above to find the probability that the $\epsilon ECR$ contains the desired $CCR$ as follows:
    \begin{align*}
        & \mathbb{P}\left(\mathbb{P}(\widehat{\ourvi} \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) ) \geq \mathbb{P}(\ourvi \leq Q_{\ourvi}(t_{\text{low}}) ) \right) \\
        &+ \mathbb{P}\left(\mathbb{P}(\widehat{\ourvi} \leq Q_{\widehat{\ourvi}}(\tau_{\text{up}}) ) \leq \mathbb{P}(\ourvi \leq Q_{\ourvi}(t_{\text{up}}) ) \right) 
        \leq 2 \delta + 2 \delta\\
        \implies &\mathbb{P}\Bigg[\left\{\mathbb{P}(\widehat{\ourvi} \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) ) \geq \mathbb{P}(\ourvi \leq Q_{\ourvi}(t_{\text{low}}) ) \right\} \\
        &\cup \left\{\mathbb{P}(\widehat{\ourvi} \leq Q_{\widehat{\ourvi}}(\tau_{\text{up}}) ) \leq \mathbb{P}(\ourvi \leq Q_{\ourvi}(t_{\text{up}}) ) \right\} \Bigg]
        \leq 4\delta
    \end{align*}
    We can then find a bound on $\mathbb{P}(CCR \subset ECR) = \mathbb{P}(\{ECR_{lb} \leq CCR_{lb}\} \cap \{ECR_{ub} \geq CCR_{ub}\})$ where $lb$ and $ub$ respectively denote the upper and lower bounds of their intervals they index, as: 
    \begin{align*}
        \mathbb{P}\Bigg(&\left\{\mathbb{P}(\widehat{\ourvi} \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) ) \geq \mathbb{P}(\ourvi \leq Q_{\ourvi}(t_{\text{low}}) ) \right\} \\
        &\cup \left\{\mathbb{P}(\widehat{\ourvi} \leq Q_{\widehat{\ourvi}}(\tau_{\text{up}}) ) \leq \mathbb{P}(\ourvi \leq Q_{\ourvi}(t_{\text{up}}) ) \right\} \Bigg)
        \leq 4\delta\\
        \iff & 1 - \mathbb{P}\bigg(\left\{\mathbb{P}(\widehat{\ourvi} \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) ) \geq \mathbb{P}(\ourvi \leq Q_{\ourvi}(t_{\text{low}}) ) \right\} \\
        &\cup \left\{\mathbb{P}(\widehat{\ourvi} \leq Q_{\widehat{\ourvi}}(\tau_{\text{up}}) ) \leq \mathbb{P}(\ourvi \leq Q_{\ourvi}(t_{\text{up}}) ) \right\} \bigg)
        \geq 1 - 4\delta\\
        \iff &\mathbb{P}\bigg(\left\{\mathbb{P}(\widehat{\ourvi} \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) ) < \mathbb{P}(\ourvi \leq Q_{\ourvi}(t_{\text{low}}) ) \right\} \\
        &\cap \left\{\mathbb{P}(\widehat{\ourvi} \leq Q_{\widehat{\ourvi}}(\tau_{\text{up}}) ) > \mathbb{P}(\ourvi \leq Q_{\ourvi}(t_{\text{up}}) ) \right\} \bigg)
        \geq 1 - 4\delta\\
        \iff &\mathbb{P} \bigg( \big(\mathbb{P}(\ourvi \leq Q_{\ourvi}(t_{\text{low}}) ), \mathbb{P}(\ourvi \leq Q_{\ourvi}(t_{\text{up}}) )\big)\\
        &\subset \left(\mathbb{P}(\widehat{\ourvi} \leq Q_{\widehat{\ourvi}}(\tau_{\text{low}}) ), \mathbb{P}(\widehat{\ourvi} \leq Q_{\widehat{\ourvi}}(\tau_{\text{up}}) )\right) \bigg)
        \geq 1 - 4\delta\\
        \iff &\mathbb{P}(CCR \subset ECR) \geq 1 - 4\delta \\
    \end{align*}
    With high probability, this states that the region of $\ourvi$ between $t_{\text{low}}$ and $t_{\text{up}}$ is contained within the region of $\widehat{\ourvi}$ between $\tau_\text{low}$ and $\tau_\text{up}$ with $B \geq \frac{1}{2\varepsilon_H^2}\ln\left( \frac{2}{\delta} \right)$ bootstrap iterations. This can be equivalently stated as
    \begin{align*}
        &\mathbb{P}(CCR \subset ECR) \geq
         1 - \delta
    \end{align*}
    with $B \geq \frac{1}{2\varepsilon_H^2}\ln\left( \frac{8}{\delta} \right)$ bootstrap iterations.
    
\end{proof}

==> supplement_files/rashomon_stability.tex <==
\begin{theorem}
    Let $\mathcal{P}_n, \mathcal{P}_n'$ represent the empirical density functions for datasets $\Dn_1, \Dn_2$ sampled i.i.d. from the same data generating process. 
    
    Let $\delta = \| \mathcal{P}_n - \mathcal{P}_n' \|_{\infty} = \sup_z |\mathcal{P}_n(z) - \mathcal{P}_n'(z)|.$ Let $\mathbf{k} \in [\phi_{min}, \phi_{max}]^p$ As $\delta$ decreases, the distance between the JRID following $\mathcal{P}_n$ and the JRID following $\mathcal{P}_n'$ decreases:
    
    \begin{align*}
        \text{ As } \delta \text{ decreases },
        \left|F_{JRID \sim \mathcal{P}_n}\left(\mathbf{k}\right) - F_{JRID \sim \mathcal{P}_n'}\left(\mathbf{k}\right) \right| 
    \end{align*}
    also decreases.
\end{theorem}

\begin{proof}
    Let $\mathcal{P}_n, \mathcal{P}_n', \mathcal{P}_n''$ represent the empirical density functions for datasets $\Dn_1, \Dn_2, \Dn_3$ sampled i.i.d. from the same data generating process. 
    
    Let $\delta_1 = \| \mathcal{P}_n - \mathcal{P}_n' \|_{\infty} = \sup_z |\mathcal{P}_n(z) - \mathcal{P}_n'(z)|$ and let $\delta_2 = \| \mathcal{P}_n - \mathcal{P}_n'' \|_{\infty} = \sup_z |\mathcal{P}_n(z) - \mathcal{P}_n''(z)|.$ Assume $\delta_1 < \delta_2.$ In other words, assume the empirical distribution $\mathcal{P}_n$ is closer to $\mathcal{P}_n'$ than it is to $\mathcal{P}_n''.$

    First, recognize that
    \begin{align*}
        F_{JRID \sim \mathcal{P}_n}\left(\mathbf{k}\right) 
        &= 
        \mathbb{E}_{\Dn \sim \mathcal{P}_n}\left[ \frac{\sum_{f \in \mathcal{R}_{\Dn}^\varepsilon} \mathbb{1}\left[\phi(f, \Dn) \leq \mathbf{k}  \right]}{|\mathcal{R}_{\Dn}^\varepsilon|} \right] \\
        &= \mathbb{E}_{\Dn \sim \mathcal{P}_n}\left[ \frac{\sum_{f \in \mathcal{R}_{\Dn}^\varepsilon} \mathbb{1}\left[\phi(f, \Dn) \leq \mathbf{k}  \right]}{|\mathcal{R}_{\Dn}^\varepsilon|} \right] \\
        &= \int_{\Dn} \left[ \frac{\sum_{f \in \mathcal{R}_{\Dn}^\varepsilon} \mathbb{1}\left[\phi(f, \Dn) \leq \mathbf{k}  \right]}{|\mathcal{R}_{\Dn}^\varepsilon|} \right] \mathcal{P}_n(\Dn) d\Dn,
    \end{align*}
    where $\int_{\Dn} d\Dn$ represents the integral over all possible datasets that could be generated from $\mathcal{P}_n$; in the case of discrete datasets, the proof still holds by replacing $\int_{\Dn} d\Dn$ with a summation over all possible $\Dn \sim \mathcal{P}_n.$ Additionally, $\mathcal{P}_n(\Dn)$ represents the density associated with observing the dataset $\Dn.$

    Now, we can represent $\left|F_{JRID \sim \mathcal{P}_n}\left(\mathbf{k}\right) - F_{JRID \sim \mathcal{P}_n'}\left(\mathbf{k}\right) \right|$ in terms of $\delta_1$

     \begin{align*}
         &\left|F_{JRID \sim \mathcal{P}_n}\left(\mathbf{k}\right) - F_{JRID \sim \mathcal{P}_n'}\left(\mathbf{k}\right) \right| \\
         = & \left| \int_{\Dn} \left[ \frac{\sum_{f \in \mathcal{R}_{\Dn}^\varepsilon} \mathbb{1}\left[\phi(f, \Dn) \leq \mathbf{k}  \right]}{|\mathcal{R}_{\Dn}^\varepsilon|} \right] \mathcal{P}_n(\Dn) d\Dn -  \int_{\Dn} \left[ \frac{\sum_{f \in \mathcal{R}_{\Dn}^\varepsilon} \mathbb{1}\left[\phi(f, \Dn) \leq \mathbf{k}  \right]}{|\mathcal{R}_{\Dn}^\varepsilon|} \right] \mathcal{P}_n'(\Dn) d\Dn \right| \\
         = & \left| \int_{\Dn} \left[ \frac{\sum_{f \in \mathcal{R}_{\Dn}^\varepsilon} \mathbb{1}\left[\phi(f, \Dn) \leq \mathbf{k}  \right]}{|\mathcal{R}_{\Dn}^\varepsilon|} \right] \mathcal{P}_n(\Dn) d\Dn -  \int_{\Dn} \left[ \frac{\sum_{f \in \mathcal{R}_{\Dn}^\varepsilon} \mathbb{1}\left[\phi(f, \Dn) \leq \mathbf{k}  \right]}{|\mathcal{R}_{\Dn}^\varepsilon|} \right] \mathcal{P}_n'(\Dn) d\Dn \right| \\
         = &\left| \int_{\Dn} \left[ \frac{\sum_{f \in \mathcal{R}_{\Dn}^\varepsilon} \mathbb{1}\left[\phi(f, \Dn) \leq \mathbf{k}  \right]}{|\mathcal{R}_{\Dn}^\varepsilon|} \right] \left(\mathcal{P}_n(\Dn) - \mathcal{P}_n'(\Dn) \right) d\Dn \right| \\
         = &\left| \int_{\Dn} \left[ \frac{\sum_{f \in \mathcal{R}_{\Dn}^\varepsilon} \mathbb{1}\left[\phi(f, \Dn) \leq \mathbf{k}  \right]}{|\mathcal{R}_{\Dn}^\varepsilon|} \right] \left(\mathcal{P}_n(\Dn) - \mathcal{P}_n'(\Dn) \right) d\Dn \right| \\
         \leq &\int_{\Dn} \left| \left[ \frac{\sum_{f \in \mathcal{R}_{\Dn}^\varepsilon} \mathbb{1}\left[\phi(f, \Dn) \leq \mathbf{k}  \right]}{|\mathcal{R}_{\Dn}^\varepsilon|} \right] \left(\mathcal{P}_n(\Dn) - \mathcal{P}_n'(\Dn) \right) \right| d\Dn \text{ by Triangle Ineq. } \\
         = &\int_{\Dn} \underbrace{\left[ \frac{\sum_{f \in \mathcal{R}_{\Dn}^\varepsilon} \mathbb{1}\left[\phi(f, \Dn) \leq \mathbf{k}  \right]}{|\mathcal{R}_{\Dn}^\varepsilon|} \right]}_{(*)} \left|  \left(\mathcal{P}_n(\Dn) - \mathcal{P}_n'(\Dn) \right) \right| d\Dn \text{ because } 0 \leq (*) \leq 1 \\
         < &\int_{\Dn} \underbrace{\left[ \frac{\sum_{f \in \mathcal{R}_{\Dn}^\varepsilon} \mathbb{1}\left[\phi(f, \Dn) \leq \mathbf{k}  \right]}{|\mathcal{R}_{\Dn}^\varepsilon|} \right]}_{(*)} \left|  \left(\mathcal{P}_n(\Dn) - \mathcal{P}_n''(\Dn) \right) \right| d\Dn \text{ because } 
         &
     \end{align*}
    
\end{proof}
